Adaptive Incentive Design

We apply control theoretic and optimization techniques to adaptively design incentives. In particular, we consider the problem of a planner with an objective that depends on data from strategic decision makers. The planner does not know the process by which the strategic agents make decisions. Under the assumption that the agents are utility maximizers, we model their interactions as a non-cooperative game and utilize the Nash equilibrium concept as well as myopic update rules to model the selection of their decision. By parameterizing the agents' utility functions and the incentives offered, we develop an algorithm that the planner can employ to learn the agents' decision-making processes while simultaneously designing incentives to change their response to a more desirable response from the planner's perspective. We provide convergence results for this algorithm both in the noise-free and noisy cases and present illustrative examples.

==> bertrand_old.tex <==
% bertrand example
In this section, we explore classical Bertrand
competition. Following~\cite{bertsimas:2015aa}, we adopt
a stylized model inspired by~\cite{berry:1994aa}. We consider a two firm
competition. Firms are assumed to have
full information and
they choose their prices $(x_1,x_2)$ to maximize their revenue
$R_i(x_1,x_2,\nu)=x_iF_i(x_1,x_2,\nu)$ where $F_i$ is the demand and $\nu$ is a normally distributed iid random variable that is common
knowledge and represents economic indicators such as GDP.



Firm $i$ has
 marginal revenue given by
\begin{align*}
    M_i(x_1,x_2)&=\log(x_i)+\theta_{i,1}^\ast x_1+\theta_{i,2}^\ast
    x_2+\theta_{ii}^\ast x_i+ \theta_{i3}+ \nu+1
    \label{eq:margrev}
\end{align*}
where in our simulations we use $\nu\sim\mc{N}(5,0.1)$ and 
$\theta_1^\ast=(-1.2,-0.5,7.5)$ and $\theta_2^\ast=(0.3,-1,1.5)$. 

When firms compete with their nominal revenue functions $R_i$, the random
variable $\nu$ changes over time causing \emph{demand shocks} which, in turn,
cause prices to shift. In our framework, we introduce a \emph{regulator} that
wants to push the prices chosen by firms towards some desired pricing level by
introducing \emph{incentives}. It is assumed that the regulator also has
knowledge of $\nu$.
We explore two variants of this problem: firms that use the myopic update rule
(i) \emph{gradient play} and (ii) \emph{approximate fictitious play}.
%We explore several variants of this problem 
%that
%help highlight the theoretical results; specifically, we consider (i) firms that
%use the myopic update rule \emph{gradient
%play} where 
We consider the nominal basis functions $\Phi_i$ to contain
radial basis functions that do not include the true basis functions. These
examples show that even if the agents are not playing according to the assumed
basis functions, it is still possible to drive the agents to a desired state
even for several classes of myopic update rules.
%and (ii)
%firms that use the myopic update rule \emph{approximate fictitious play}

In the gradient play case, each firm's price evolves according to 
\begin{equation}
x_i^{k+1} = x_i^k + \gamma_k (M_i(x_1^k, x_2^k) + \langle \Psi_i(x_i^k, x_{-i}^k), \alpha_i^{k} \rangle),
\end{equation}
and, in the approximate fictitious play case, each firm's price evolves
according to
\begin{equation}
    x_i^{k+1} = x_i^k + \gamma_k (M_i(x_1^k, \bar{x}_2^{(l,k)}) + \langle
    \Psi_i(x_1^k, \bar{x}_2^{(l,k)}), \alpha_i^{k} \rangle),
\end{equation}
where $\gamma_k$ is their learning rate and $\bar{x}_i^{(l,k)}$ is the average
over the history from $l$ to $k$ with $0\leq l\leq k$.
For our simulations, we choose $\gamma_k$ to ensure stability of the process.

 



==> incent_alg.tex <==
%\subsection{Algorithm---Nash Play}
  \label{sec:alg}
Now that we have formulated the utility learning problem and the incentive
design problem at each iteration, we formulate the algorithm for
estimating the parameters and designing the incentive mechanism. 


\begin{algorithm}[t]
  \caption{Online Utility Learning and Incentive Design}
  \label{alg:nash}
  \begin{algorithmic}[1]
%    \item  \textbf{If} Nash--play \textbf{then}
%  \item   $\quad$Choose $\alpha_i^{(0)}\in \mb{R}^{m_i}$ for each $i\in\pl$
%    \item $\quad$$k\leftarrow0$
%%  \item    $\quad$Issue incentive mapping $\gamma_i(\x)=\Psi_i(\x)^T\alpha_i^{(0)}$
 \item \textbf{If} myopic--play \textbf{then} receive $\xx{0}$
 %\item $\quad$ Receive $\xx{0}$
%  \item$\quad$Choose $\alpha_i^{(0)}\in \mb{R}^{m_i}$ for each $i\in\pl$
%  \item $\quad$$k\leftarrow 0$
 
\item   Choose $\ala{0}{i}\in \mb{R}^{m_i}$, $\tit{i}{0}\in \Theta_i$ for each $i\in\pl$
%\item   Choose $\ala{0}{i}\in \mb{R}^{m_i}$ for each $i\in\pl$
    \item Issue incentive mapping
      $\gamma_i(x)=\Psi_i(x)^T\ala{0}{i}$
  \item $k\leftarrow 0$
 % \item \textbf{for} {$k=0,2, \ldots$} \textbf{do}
 \item \textbf{do}
  \item $\quad$ \textbf{for} {$i=1, \ldots, \n$} 
  \item $\qquad$ Receive observation $y^{k+1}_i$ and incur loss
    $\ell(\tit{i}{k})$
%  \item $\qquad$ \textbf{utility learning}:
    \item $\qquad\quad$\textbf{If} Nash--play \textbf{then}
    \item  $\qquad\qquad$ $\tit{i}{k+1}=P_{\tit{i}{k}}^{k+1}\left( \eta_k\nabla
    \ell(\tit{i}{k}) \right)$ 
      \item $\qquad\qquad$ Choose
    $\ala{k+1}{i}\in\mc{A}(\tu{k+1}, x^d, \y^d)$ [or
    $\mc{A}_s(\tu{k+1}, x^d, \y^d)$]
    \item $\quad\qquad$\textbf{If} myopic--play \textbf{then}
    \item  $\qquad\qquad$ $\tit{i}{k+1}=P_{\tit{i}{k}}\left( \eta_k\nabla
    \ell(\tit{i}{k}) \right)$
    \item $\qquad\qquad$ Choose $\ala{k+1}{i}\in\mc{A}_m(\tu{k+1}, \xx{k}, x^d, \y^d)$
%  \item $\qquad$ \textbf{incentive design}: 
%  \item $\qquad\quad$\textbf{If} Nash--play \textbf{then}
%  \item $\qquad\qquad$ Choose
%    $\ala{k+1}{i}\in\mc{A}(\tu{k+1}, x^d, \y^d)$ [or
%    $\mc{A}_s(\tu{k+1}, x^d, \y^d)$]
%  \item $\quad\qquad$\textbf{If} myopic--play \textbf{then}
%  \item $\qquad\qquad$ Choose $\ala{k+1}{i}\in\mc{A}_m(\tu{k+1}, \xx{k}, x^d, \y^d)$
% %(resp. $\mc{A}_s(\theta^{(k+1)}, \x^d, \y^d)$)
 \item $\qquad$ Issue incentive mapping $\gamma_i(x)=\Psi_i(x)^T\ala{k+1}{i}$
  \item $\quad$ \textbf{end for}
  \item $\quad$ $k\leftarrow k+1$
 \item \textbf{end do}
  \end{algorithmic}
\end{algorithm}

%Again, it is
%straightforward to find an $\ala{k+1}{i}$ by solving the optimization
%problem posed in~\eqref{eq:lsq-alpha-myop}.

Suppose the coordinator has optimized its cost $f_c(x,\y)$ to determine $x^d$
and $\y^d$. If the agents are playing according to Nash, then suppose that Assumption~\ref{ass:nash-1}
(Assumption~\ref{ass:nash-1-mod}, respectively) holds. On the other hand, if the
agents are playing myopically, then suppose that
Assumption~\ref{ass:myopic} holds. Then, following
Algorithm~\ref{alg:nash}, the coordinator has a procedure for updating the parameter
estimates for each agent's cost function and for choosing the incentive
mechanism given the estimated parameters. In the {\nplay} case, the planner must use
the time varying prox{\ds}mapping $P^{k+1}_{\tit{i}{k}}$ where in the
{\mplay} case they use $P_{\tit{i}{k}}$. 
%Note that by replacing
%$\mc{A}(\theta^{(k+1)}, x^d, \y^d)$ in line $17$ of Algorithm~\ref{alg:nash}
%with $\mc{A}_s(\theta^{(k+1)}, x^d, \y^d)$, allows the coordinator to choose an incentive
%such that the estimated response is a stable, non--degenerate differential Nash
%equilibrium. 
%At iteration $k$, we have data
%$\{\xx{t}\}_{t=0}^k$ and $\{\al{t}\}_{t=0}^k$. 



==> incent_noise.tex <==
\label{sec:noise}
In this section, we will use the unified framework that describes both the case
where the agents play according to Nash and where the agents play myopically.

We will again consider the case where the agents have multiple inputs,
$X_i\subset \mb{R}^{p_i}$, $p_i\geq 1$ for each $i\in\pl$;
  however, we will make the simplifying assumption that there
  is a different set of basis functions for each input. 
  In particular, 
  suppose each player's input is denoted by $x_i=(x_{i,1},
  \ldots, x_{i,p_i})$ and we assume that each input has its own set of basis
  functions $\{\phi_{i,l,j}\}_{j=1}^{m_{i,l}}$, $l\in\{1, \ldots, p_i\}$ and
  $m_{i,l}$ denotes the dimension of $\ts_{i,l,j}$. 
  %Define
  %$\Phi_{i,l}=[\phi_{i,l,1}(\x)\ \cdots\ \phi_{i,l,m_{i,l}}]^T$. 
  %With
  %$\xi_{i,l}^t=D_{i_l}\Phi_{i,l}(\x^{(t)})$, 
  We can state \eqref{eq:y} as
  \begin{equation}
    \bmat{y_{i,1}^{k+1}\\ \vdots\\ y_{i,p_i}^{k+1}}=\bmat{(\xi_{i,1}^k)^T 
    &\cdots & 0\\
    % 0&(\xi_{i,2}^t)^T&0 &\cdots &0\\
     \vdots&  \ddots &\vdots\\
     0 &  \cdots  & (\xi_{i,p_i}^k)^T}\bmat{\ts_{i,1}\\ \vdots \\
     \ts_{i,p_i}} %+\bmat{w_{i,1}^{t+1}\\ \vdots\\ w_{i,p_i}^{t+1}}
    \label{eq:multi-in-1}
  \end{equation}
  In this case,   observations decouple and hence,
  the estimation for each set of parameters decouples. In this case, 
   each $\tit{i,l}{k}$ is updated  according to
  Algorithm~\ref{alg:nash} independently from the others.
  Since the notation is
  cumbersome and the details straightforward, we drop the additional index for
  each input. That is, instead of considering the update of our estimate of
  $\ts_{i,l}$ in Algorithm~\ref{alg:nash}, we simply consider the update of
  $\ts_i$ and note that due to the independence of the parameters for each
  input, that we could apply the update to each $\ts_{i,l}$.

  In addition, we will consider \emph{noisy} updates given by
%That is, we will denote each agent's update by $y_i^{t+1}$ where
\begin{equation}
  y_i^{k+1}=(\xi_i^k)^T\ts_i + w_i^{k+1}
  \label{eq:update-n}
\end{equation}
for each $i\in\pl$ where $w_i^{k+1}$ is an indepdent, identically distributed (i.i.d) 
%zero mean
real stochastic process defined on a probability space $(\Omega, F, P)$ adapted
to the sequence of increasing sub-$\sigma$--algebras $(F_k, k\in \mb{N})$, where
$F_k$ is the $\sigma$--algebra generated by the set $\{y_i^t,
\ala{t}{i},
w_i^t, t\leq k\}$ and
such that the following hold:
%$\mb{E}[(w_i^{t})^2]=\sigma_i^2$.
\begin{equation}
  \mb{E}[w_i^{k+1}| F_k]=0\  \forall k;\  \mb{E}[(w_i^{k+1})^2| F_k]=
  \sigma^2>0 \  \text{a.s.}\  \forall k; \ \sup_t \mb{E}[(w_i^{k+1})^4| F_k]<+\infty\ \text{a.s.}
  \label{eq:zeromean}
\end{equation}
%and
%\begin{equation}
%  \mb{E}[(w_i^{t+1})^2| F_t]= \sigma^2>0 \ \ \text{a.s.}\  \forall\  t.
%  \label{eq:var}
%\end{equation}
%and
%\begin{equation}
%  \sup_t \mb{E}[(w_i^{t+1})^4| F_t]<+\infty\ \text{a.s.}
%  \label{eq:fourthorder}
%\end{equation}
 Note that $F_k$ is also the $\sigma$--algebra generated by
$\{y_i^t, \xi_i^t, t\leq k\}$ since $w_i^k$ can be deduced from $y_i^k$ and
$\xi_i^{k-1}$ through the relationship
$w_i^{k}=y_i^k-(\xi_i^{k-1})^T\ts_i$~\cite{kumar:1986aa}.

For simplicity, in this section we will assume that $X_i\subseteq\mb{R}^{p_i}$
with $p_i>1$ and that there is a different set of basis functions for each input as
described in~\eqref{eq:multi-in-1}.  We will also drop the additional index
corresponding to each input for each player since the same analysis can be
applied to each of the inputs seperately. That is, instead of considering $p_i$
different observations 
 $y_{i,l}^{k+1}=(\xi_{i,l}^k)^T\ts_{i,l} + w_{i,l}^{k+1}$ for
$l\in\{1, \ldots, p_i\}$
we will perform the analysis for $y_i^{k+1}=(\xi_i^k)^T\ts_i + w_i^{k+1}$ and
simply note that the same analysis holds for each input without carrying around
the extra index $l$.
%Please refer back to Section~\ref{subsec:UL-nash} for the Nash case and
%Section~\ref{subsec:UL-myopic} for the myopic case.
%
%We address the scenario in which the agents' updates are \emph{noisy}. 

\begin{theorem}
  Suppose that for
  each $i\in\pl$, 
  $\{w_i^{k}\}$ satisfies \eqref{eq:zeromean} and that Algorithm~\ref{alg:nash},
  with prox--mapping $P_\theta$ associated with $\beta$ (modulus $\nu$), is 
  {persistently exciting} and stable.
%  . Furthermore,
%  suppose that a central planner follows Algorithm~\ref{alg:nash} for utility
%  learning and incentive design using the 
% prox--mapping $P_\theta$ associated with $\beta$ (modulus $\nu$)
%  and that the algorithm is {persistently exciting} and stable. 
Let the 
  step--size $\eta_k$
  be selected such that %$\sum_{t=1}^\infty \eta_t=\infty$,
  $\sum_{k=1}^\infty\eta_k^2<\infty$ and
  $\eta_k-\frac{\eta_k^2}{2\nu}\tilde{c}_1>0$
  %for some $\vep$ such
  %that $0<\vep <\frac{1}{2c_2}$ and 
  where
   $0<\tilde{c}_s<\infty$ is such that $\|\xi_i^k\|_\ast^2\leq \tilde{c}_s$.
   %and
   %$c_2=\min_{i\in\pl}c_{i,2}$.
  Then, for each $i\in\pl$, 
  $V_k(\ts_i)$ converges
  {a.s}.
  Furthermore, if the sequence
  $\{r_k\}$ where $r_k=(\eta_k-\frac{\eta_k^2}{2\nu}\tilde{c}_s)^{-1}$ is a non-decreasing,
  non-negative sequence such that $r_k$ is $F_k$ measurable and there
  exists constants $0<K_1, K_2<\infty$ and $0<{T}<\infty$ such that
  \begin{equation}\textstyle
    \frac{1}{k}r_{k-1}\leq
  K_1+\frac{K_2}{k}\sum_{t=0}^{k-1}(y_i^{t+1}-(\xi_i^{t})^T\tit{i}{t}-w_i^{t+1})^2,
  \ \ \forall  \ k\geq {T},
  \label{eq:rbound}
\end{equation}
then 
\begin{equation}\textstyle
  \lim_{k\rar\infty}
  \frac{1}{k}\sum_{t=0}^{k-1}\mb{E}[(y_i^{t+1}-(\xi_i^{t})^T\tit{i}{t})^2|
F_t]=\sigma^2\ \ \text{a.s.}
\label{eq:errorcon-yy}
\end{equation}
  If, in addition,  
  %\begin{equation}
  $\sup_k \mb{E}[(w_i^{k+1})^4| F_k]<+\infty$ a.s.
  %\label{eq:fourthorder}
%\end{equation}
then
\begin{equation}\textstyle
  \lim_{k\rar\infty}
\frac{1}{k}\sum_{t=0}^{k-1}(y_i^{t+1}-(\xi_i^{t})^T\tit{i}{t})^2=\sigma^2\ \ \text{a.s.}
\label{eq:errorcon-y}
\end{equation}
  %If, in addition,
  %$\lim_{t\rar\infty}\left(\eta_t-\frac{\eta_t^2}{2\nu}\tilde{c}_1\right)^{-1}=\infty$,
  %then 
  %\begin{equation}
  %  \lim_{T\rar\infty}\left( \eta_T-\frac{\eta_T^2}{2\nu}\tilde{c}_1
  %  \right)\sum_{t=1}^T\left( \mb{E}[y_i^{t+1}-(\xi_i^t)^T\theta_i^{(t)}| F_t]
  %  \right)^2=0 \ \ \text{a.s.}
  %  \label{eq:limeq}
  %\end{equation}
  \label{thm:noise}
\end{theorem}
The proof follows a similar technique to that presented in~\cite[Chapter
13.4]{kumar:1986aa}; hence, we leave it to Appendix~\ref{app:proofs}. 

%Before we move on, let us remark on the assumptions of Theorem~\ref{thm:noise}.
%We can make some modificaitons to the assumptions in order to simplify some of the
%ones that are more difficult to check. In particular, if we assume that each
%$\Theta_i^{(t)}$ is bounded, then by letting $r_t=\eta_t^{-1}$

Let us state an alternative version of the above theorem after which we will make comments
on the differences between the assumptions. 
\begin{theorem}
  Suppose that for
  each $i\in\pl$, 
  $\{w_i^{k}\}$ satisfies \eqref{eq:zeromean} and that Algorithm~\ref{alg:nash},
  with prox--mapping $P_\theta$ associated with $\beta$ (modulus $\nu$), is 
  {persistently exciting} and stable. Let the 
  step--size $\eta_k$
  be selected such that %$\sum_{t=1}^\infty \eta_t=\infty$,
  $\sum_{k=1}^\infty\eta_k^2<\infty$ and
  $\eta_k>0$
  %for some $\vep$ such
  %that $0<\vep <\frac{1}{2c_2}$ and 
  where
   $0<\tilde{c}_s<\infty$ is such that $\|\xi_i^k\|_\ast^2\leq \tilde{c}_s$.
   %and
   %$c_2=\min_{i\in\pl}c_{i,2}$.
  Then, for each $i\in\pl$, 
  $V_k(\ts_i)$ converges
  a.s.
  Furthermore, if %suppose that each $\Theta_i^{t}$ is bounded and that 
  the sequence
  $\{r_k\}$ where $r_k=(\eta_k)^{-1}$ is a non-decreasing,
  non-negative sequence such that $r_k$ is $F_k$ measurable and there
  exists constants $0<K_1, K_2<\infty$ and $0<{T}<\infty$ such that
  \begin{equation}\textstyle
    \frac{1}{k}r_{k-1}\leq
  K_1+\frac{K_2}{k}\sum_{t=0}^{k-1}(y_i^{t+1}-(\xi_i^{t})^T\tit{i}{t}-w_i^{t+1})^2,
  \ \ \forall  \ k\geq {T},
  \label{eq:rbound-22}
\end{equation}
then 
\begin{equation}\textstyle
  \lim_{k\rar\infty}
  \frac{1}{k}\sum_{t=0}^{k-1}\mb{E}[(y_i^{t+1}-(\xi_i^{t})^T\tit{i}{t})^2|
F_t]=\sigma^2\ \ \text{a.s.}
\label{eq:errorcon-2}
\end{equation}
  If, in addition, 
  %\begin{equation}\textstyle
  $\sup_k \mb{E}[(w_i^{k+1})^4| F_k]<+\infty$ {a.s.}
 % \label{eq:fourthorder-2}
%\end{equation}
then
\begin{equation}\textstyle
  \lim_{k\rar\infty}
\frac{1}{k}\sum_{t=0}^{k-1}(y_i^{t+1}-(\xi_i^{t})^T\tit{i}{t})^2=\sigma^2\ \ \text{a.s.}
\label{eq:errorcon-22}
\end{equation}
  \label{thm:noise-p}
\end{theorem}
%Note that added the assumption that each $\Theta_i^{t}$ is bounded and the
%modified
% assumption on the sequence $r_t$. 
 The proof follows the same argument as the
 proof of Theorem~\ref{thm:noise}.
%\begin{proof}
%    The proof is essentially the same as above with some minor modifications.
%    %follows a similar technique to that presented in~\cite[Chapter
%  %13.4]{kumar:1986aa}.
% % Since $\ell(\theta)$ is convex, we have
% % \[\ell(\tit{i}{t})-\ell(\theta_i)\leq \nabla
% % \ell(\theta_i)(\ta{i}-\tit{i}{t})\]
% Starting from Lemma~\ref{lem:tvpmaps}, we have
% \begin{align}
%   \mb{E}[V_{t+1}(\ts_i)|F_t]&\leq
%   V_t(\ts_i)-\eta_t(\ts_i-\tit{i}{t})^T\xi_i^t(\mb{E}[y_i^{t+1}-(\xi_i^t)^T\tit{i}{t}|F_t])\notag\\
%   &\qquad+\frac{\eta_t^2}{2\nu}\|\xi_i^t\|_\ast^2\left((\mb{E}[y_i^{t+1}-(\xi_i^t)^T\tit{i}{t}|F_t]
%    )^2+\sigma^2\right)\\
% %   &\leq V_t(\theta_i)-\eta_t\left(
% %   (\theta_i-\theta_i^{(t)})^T\xi_i^t-\frac{\eta_t}{2\nu}\|\xi_i^t\|_\ast^2\mb{E}[y_i^{t+1}-(\xi_i^t)^T\theta_i^{(t)}|F_t]
% %   \right)\notag\\
% %   &\qquad
% %   \cdot\mb{E}[y_i^{t+1}-(\xi_i^t)^T\theta_i^{(t)}|F_t]+\frac{\eta_t^2}{2\nu}\|\xi_i^t\|_\ast^2\sigma^2\\
%    &\leq V_t(\ts_i)-
%    \eta_t \left( \mb{E}[y_i^{t+1}-(\xi_i^t)^T\tit{i}{t}|F_t]
%    \right)^2\notag\\
%    &\qquad+\frac{\eta_t^2}{2\nu}\|\xi_i^t\|_\ast^2\left(\sigma^2+(\mb{E}[y_i^{t+1}-(\xi_i^t)^T\tit{i}{t}|F_t])^2
%    \right)
%%    &\leq  V_t(\theta_i)-\left(
%%    \eta_t-\frac{\eta_t^2}{2\nu}\tilde{c}_1 \right)\left( \mb{E}[y_i^{t+1}-(\xi_i^t)^T\theta_i^{(t)}|F_t]
%%    \right)^2+\frac{\eta_t^2}{2\nu}\tilde{c}_1\sigma^2
%   \label{eq:noiseeq}
% \end{align} 
% Hence, since $\Theta_i^{t}$ is bounded along with the stability assumption, we have that there exists some
% constant $b$ such that $\mb{E}[y_i^{t+1}-(\xi_i^t)^T\tit{i}{t}|F_t]<b$. 
%This gives us that 
%\eq{eq:r}{\mb{E}[V_{t+1}(\ts_i)|F_t]\leq V_t(\ts_i)-
%    \eta_t \left( \mb{E}[y_i^{t+1}-(\xi_i^t)^T\tit{i}{t}|F_t]
%    \right)^2+\frac{\eta_t^2}{2\nu}\|\xi_i^t\|_\ast^2\left(\sigma^2+b^2
%    \right)}
%
% By the assumptions that $\eta_t>0$ and
% $\sum_{t=1}^\infty\eta_t^2<\infty$, we can apply the almost supermartingale
% convergence theorem (Theorem~\ref{thm:asmc}) to get that  
% \begin{equation}\textstyle
% \sum_{t=1}^\infty 
%    \eta_t \left( \mb{E}[y_i^{t+1}-(\xi_i^t)^T\tit{i}{t}|F_t]
%    \right)^2<\infty\ \ \text{a.s.}
%    \label{eq:sumit-p}
%  \end{equation}
%     and that $V_t(\ts_i)$
%    converges almost surely. 
%  
%    The remainder of the proof follows exactly what was shown for
%    Theorem~\ref{thm:noise} only with $r_t=\eta_t^{-1}$; hence, we refer the reader to its proof.
%    %which is to say that $\|\theta_i^{(t)}-\theta_i\|^2$
%    %converges almost surely.
% \end{proof}
 \begin{remark}
   Let us remark on the difference between Theorem~\ref{thm:noise} and
 Theorem~\ref{thm:noise-p}. The simplified assumptions on the step--size
 $\eta_k$ allow for us to find choices for $\eta_k$ for which it is much easier
 to check if condition~\eqref{eq:rbound-22} is satisfied. For instance, the
 step--size $\eta_k=k^{-1}$ trivially satisfies \eqref{eq:rbound-22} and
 $\sum_{k}\eta_k^2<\infty$. Further, the rate at which $r_t$ increases is much
 slower since $r_k=\eta_k^{-1}$ instead of
 $r_k=(\eta_k-\frac{\eta_k^2}{2\nu}\tilde{c}_s)^{-1}$. This is desirable and
 is, in part, the purpose of \eqref{eq:rbound-22}, i.e. to ensure that the rate
 that $r_k$ grows is proportionally upper bounded by the average error. 
% The
%drawback to Theorem~\ref{thm:noise-p} is the additional assumption that
% $\Theta_i^{t}$ is bounded. 
 \end{remark}
 \begin{corollary}
   Suppose the assumptions of Theorem~\ref{thm:noise} (or
   Theorem~\ref{thm:noise-p}) hold with the exception that in
   Algorithm~\ref{alg:nash}, we use the prox--mapping $P_\theta$ associated with
   $\beta(\theta)=\frac{1}{2}\|\theta\|_2^2$ (modulus $\nu=1$). Then 
   $V_k(\ts_i)=\frac{1}{2}\|\ts_i-\tit{i}{k}\|_2^2$ converges a.s.
  \label{cor:tscon}
 \end{corollary}
%\textcolor{red}{need to make remarks on $\eta_t$.
%\begin{itemize}
%  \item first, we could change the situation so that we assume that $\Theta$ is
%    bound for each $t$. Then, we can argue that with $r_t=\eta_t^{-1}$ and the
%    other assumptions we get convergence. The here we have a much simpler choice
%    for $\eta_t$ and we dont have $\eta_t$ decreasing \emph{too rapidly} which
%    is the interpretation of (3.6.5) (i.e. we want $\{r_t/T\}$ to be bounded but
%    we dont want it to increase too rapidly either as compared to the error.
%  \item second we could choose simple step sizes in this case that trivially
%    satisfy the bound in (3.6.5) for instance we could choose
%    $\eta_t=\frac{1}{t}$. this trivially satisfies that bound and is something
%    we can easily check whereas otherwise this bound would be hard to check.
%  \item also add proof of proposition
%\end{itemize}}
%\begin{remark}

In the myopic--play case,
%---that is where
%  $\bx{i}{k+1}=\td{\Phi}_i(\xx{k})^T\ts_i+\td{\Psi}_i(\xx{k})^T\ala{k}{i}$---
  as
  a consequence of \eqref{eq:errorcon-yy}, we expect that the average mean square error
  between the desired response $x^d$ and the actual response $\xx{k}$
  converges to $\sigma^2$ a.s. Indeed, \eqref{eq:errorcon-yy} of
  Theorem~\ref{thm:noise}---or~\eqref{eq:errorcon-2} of
  Theorem~\ref{thm:noise-p}---imply  
\begin{align}\textstyle
%  &\lim_{T\rar\infty}
%  \frac{1}{T}\sum_{t=0}^{T-1}\mb{E}[(u_i^{(t+1)}-\td{\Psi}_i(u^{(t)})^T\alpha^{(t)}+w_i^{t+1}-u_i^d+\td{\Psi}_i(u^{(t)})^T\alpha^{(t)})^2|
%F_t]\\
%&\quad=
\lim_{k\rar\infty}\frac{1}{k}\sum_{t=0}^{k-1}\mb{E}[(\bx{i}{t+1}+w_i^{t+1}-x_i^d)^2|
F_t]
=\sigma^2\ \ \text{a.s.}
\end{align}
    Furthermore, note that we have designed
    $\ala{t+1}{i}$ to satisfy $\gamma_i(x^d)=\Psi(\xx{t})^T\ala{t+1}{i}$
  (or at the very least approximately if we solve the optimization problem posed
  in \eqref{eq:lsq-alpha-myop} as opposed to explicitly solving the linear
  system of equations). 
  
  On the other hand, in the Nash--play case, it is
  difficult to say much about the observed Nash equilibrium except in
  expectation. In particular, we can consider a modified version of
  Theorem~\ref{thm:nash-bound} where we consider the differential game form in
  expectation, i.e.~at iteration $k$,  the
  differential game form for the induced game is %given by
  \eq{eq:modomega}{\textstyle
  \td{\omega}(\theta,
  x)=\sum_{i=1}^\n\mb{E}\left[D_i\Phi_i(x)^T\theta_i+D_i\Psi_i(x)^T\ala{k}{i}+w_i^{k+1}|
  F_{k-1}\right].
%  \mb{E}\left[\sum_{i=1}^{\n}\sum_{l=1}^{p_i}\left(\sum_{j=1}^{m_i}D_{i_l}\phi_{i,j}(\x)\theta_{i,j}+\sum_{k=1}^{n_i}D_{i_l}\psi_{i,k}(\x)\alpha_{i,j}\right)
%   d\x_i^l\right]
  }
%  Before, we knew that $D_2\omega(\ts, x^d)$ was an isomorphism since $x^d$
%  is a non--degenerate differential Nash equilibrium. Here, in order to apply
%  the Implicit Function Theorem as in  Theorem~\ref{thm:nash-bound}, we need
%  that $D_2\td{\omega}(\ts, x^d)$ is an isomorphism. Hence, we have the
%  following result.
  
\begin{proposition}
  Suppose that $D_2\td{\omega}(\theta, x^d)$ is an isomorphism. There exists an
  $\epsilon>0$, such that for all $\tu{t}\in B_\epsilon(\ts)$,
   \begin{equation}
     % \|\x^{(t+1)}-\x^d\|\leq C\cdot M\|\theta^{(t+1)}-\theta\|
     \|x^{\ast}-x^d\|\leq  \left( \sup_{0\leq \lambda\leq 1}\|Dg(
     (1-\lambda)\ts+\lambda\tu{t})\| \right)\|\tu{t}-\theta\|
      \label{eq:bound-vep-noise}
    \end{equation}
    where
    %\begin{equation}\textstyle
      $Dg(\ts)=-(D_2\td{\omega})^{-1}(\ts, x^d)\circ D_1\td{\omega}(\ts, x^d)$.
    %  \label{eq:DG-noise}
    %\end{equation}
    and $x^\ast$ is a Nash equilibrium of the incentivized game  $(\fg{1}(x;
    \ts_1), \ldots, \fg{\n}(x, \ts_\n))$ with
    $\gamma_i(x)=\Psi_i(x)^T\ala{t}{i}$ for each $i\in\pl$. 
Furthermore, 
    if $\|Dg(\ts)\|$
 is uniformly bounded by $M>0$ on $B_{\epsilon}(\ts)$, then
    \begin{equation}
     % \|\x^{(t+1)}-\x^d\|\leq C\cdot M\|\theta^{(t+1)}-\theta\|
     \|x^{\ast}-x^d\|\leq  M\|\tu{t}-\ts\|
      \label{eq:bound-vep-n}
    \end{equation}
    \label{prop:noisynashbdd}
\end{proposition}
%As before, if the cost functions are convex and the incentive parameter $\alpha^{(t)}$ is chosen such
%that $u^{d}$ is a non--degenerate differential Nash equilibrium of the
%incentivized game and such that each $\fg{i}$ is convex,
%then we can replace $u^\ast$ with $u^{(t+1)}$ since $u^{(t+1)}$ is unique. 
%  \textcolor{red}{put in part about expected value theorem (need $E[\omega]$ to
%  be differentiable), also add in proof of contracting proximal map, and
%  consider mentioning the constant value version of the IFT}

To apply Proposition~\ref{prop:noisynashbdd} we need
that the parameter estimate $\tu{t}$ converges to the true parameter value
$\ts$. One of the consequences of Theorem~\ref{thm:noise} (respectively
Theorem~\ref{thm:noise-p}) is that $V_t(\ts_i)$ converges a.s.~and
as a consequence of Corollary~\ref{cor:tscon}, $\|\ts_i-\tit{i}{t}\|_2^2$
converges a.s. If the value it converges a.s. to is less than $\epsilon$,
then Proposition~\ref{prop:noisynashbdd} would guarantee that a Nash
equilibrium of the incentivized game is near the desired
non--degenerate differential Nash equilibrium in expectation. We leave further
exploration of the convergence of the parameter estimate $\tu{t}$ as
future work. 

The results of Theorem~\ref{thm:noise}  imply  that the average mean square error
  between 
  the observations and the predictions converges to $\sigma^2$ a.s.~and
  if we recall, the observations are derived from noisy versions of the
  first--order conditions for Nash. Indeed,
%  i.e.~we have the observation
%  $y_i^{t+1}=(\xi_i^t)^T\ts_i+w_i^{t+1}=D_i\Phi_i(\xx{t+1})^T\ts_i+w_i^{t+1}$
%  and its predicted value
%  $(\xi_i^t)^T\tit{i}{t}=D_i\Phi_i(\xx{t+1})^T\tit{i}{t}=-\D_i\Psi_i(\xx{t+1})^T\ala{t}{i}.$
%  Thus,  
we have shown that
  \eq{eq:congverg1}{\textstyle\lim_{k\rar\infty}
  \frac{1}{k}\sum_{t=0}^{k-1}\mb{E}[(D_i\Phi_i(\xx{t+1})^T\ts_i+w_i^{t+1}+\D_i\Psi_i(\xx{t+1})^T\ala{t}{i})^2|
  F_t]=\sigma^2\ \ \text{a.s.}}
or, equivalently,
\eq{eq:converge2}{\textstyle\lim_{k\rar\infty}
\frac{1}{k}\sum_{t=0}^{k-1}\mb{E}[(D_i\Phi_i(\xx{t+1})^T(\ts_i-\tit{i}{t})+w_i^{t+1})^2|
F_t]=\sigma^2\ \ \text{a.s.}}

%Depending on the noise characteristics, particularly the magnitude of
%$\sigma^2$, we may be able to argue that the agents are playing an $\vep$--Nash
%equilibrium by using a similar argument to that in Theorem~\ref{thm:nash-bound}.
%The details are left for future work. In the concluding chapter, remarks will be
%made regarding the many open questions this work has exposed including making
%connections between traditional tools of adaptive control and online learning.
%which we will now make remarks about in the context of the previous sections of
%this chapter.
%Furthermore, we will cover the

% \end{remark}
%\begin{remark}[Connections to Adaptive Control and Online Learning]
%  There are some not so subtle connections to the adaptive control literature.
%  In particular, if in the myopic--play case the entries of
%  $\td{\Phi}_i(u)$ and $\td{\Psi}(u)$ are linear in $u_i$, then the problem can
%  easily as a classical linear adaptive control problem~\cite[Chapter 10 \& 13]{kumar:1986aa}.  The
%  Nash--play case has some distinctions in that the actual response is defined
%  implicitly through the first{\ds} and second{\ds}order conditions for local Nash
%  equilibria and is therefore new. 
%
%  Similarly, if we consider only the problem of estimating $\theta$, then both
%  the Nash--play case and the myopic--play case, even with nonlinearities in the
%  observation updates,
%  can be cast as online estimation
%  problem~\cite[Chapter 3 \& 8]{goodwin:1984aa} with the added difference
% that in the present work
%  we did not select specific step--sizes. For example, 
%%  \[\td{\Phi}_{i}(u)=[\td{\phi}_{i,1}(u)\ \cdots \td{\phi}_{i,m_i}(u)]\
%%  \text{ and } \td{\Psi}_{i}(u)=[\td{\psi}_{i,1}(u)\ \cdots \td{\psi}_{i,n_i}(u)]\]
%%  where $\td{\phi}_{i,j}(u)$ and $\td{\psi}_{i,j}(u)$ are linear in $u_i$
%%  the entire theory developed for the mu
%if we make specific choices for the step--size $\eta_t$ such as
%%$\eta_t=\frac{a}{c+\|\xi_i^t\|_\ast^2}$, then the assumptions of
%%Theorem~\ref{thm:noise} can be streamlined. For instance, using the $2$--norm so
% \[\eta_t=\frac{a}{c+\|\xi_i^t\|_2^2},\] the update scheme for
%$\theta^{(t)}_i$ reduces to the projection algorithm.
%Alternatively, if $\eta_t=\frac{\mu}{r_k}$ where
%$r_k=1+\sum_{t=0}^k(\xi_i^t)^T\xi_i^t$ and $\mu>0$, then updates for $\theta$
%follow the
%algorithm introduced in~\cite{kumar:1986aa}. 
%
%It is interesting
%to note that the persistence of excitation
%condition required to ensure convergence is informed by the choice of
%step--size. This is explored extensively in~\cite[Chapter 3.4]{goodwin:1984aa}.
%However, because the conditions required for persistence of excitation depend on
%the data received at each time step (and this is true of
%Definition~\ref{def:persist} as well), it is difficult to check when an
%algorithm is persistently exciting a priori.
%In~\cite{sastry:1989aa} and~\cite{boyd:1986aa}, necessary and sufficient
%conditions are provided for persistence of excitation for model reference
%adaptive control. We are exploring extensions for the problems described in
%this chapter.
%
%Our approach here is to try to remove the dependence of the results on the
%choice of step--size and to generalize to arbitrary choice of proximal mapping.
%This approach is similar to that which is done in 
%the online learning literature~\cite{raginsky:2010aa,
%nemirovski:2009aa}. The perceived gain is that this flexibility can allow for
%the proximal mapping to be informed by the geometry of the constraint set
%(feasible parameter space) thereby resulting in improved convergence rates. 
%
%There are a number of open questions in this area.
%For instance, in order to ensure we have estimated parameters that correspond
%to a game with stable, non--degenerate differential Nash equilibria requires
%having a constraint set defined by semi--definite constraints, i.e.
%\eq{eq:thetanew}{
%\Theta_i^k=\{\theta_i\in \Theta_i|\ D^2\Phi(u^{(t)}, \theta_i)+D^2\Psi(u^{(t)},
%\alpha^{(t-1)})\geq 0, \ t\in\{1, \ldots, k\}\}\subset \Theta_i}
%where $D^2\Phi$ and $D^2\Psi$ are defined in \eqref{eq:dsqphi} and \eqref{eq:dsqpsi}
%respectively. Given that proximal maps informed by the geometry---as the
%example in Remark~\ref{rem:geom} indicates---one interesting direction for future research is
%to investigate proximal maps that are 
%%Is there a
%%proximal map that is 
%informed by the geometry of a the positive semi--definite
%cone of matrices.
%%that leads to better, in some sense, convergence properties? We
%%leave such questions as future work.
%%which is commonly used in the adaptive
%%control literature and estimation~\cite{raginsky:2010aa}and some remarks on
%%  connection to adative control
%\end{remark}



==> incent_noise2.tex <==
\label{sec:noise}
In this section, we will use the unified framework that describes both the case
where the agents play according to Nash and where the agents play myopically.

We will again consider the case where the agents have multiple inputs,
$X_i\subset \mb{R}^{p_i}$, $p_i\geq 1$ for each $i\in\pl$;
  however, we will make the simplifying assumption that there
  is a different set of basis functions for each input. 
  In particular, 
  suppose each player's input is denoted by $x_i=(x_{i,1},
  \ldots, x_{i,p_i})$ and we assume that each input has its own set of basis
  functions $\{\phi_{i,l,j}\}_{j=1}^{m_{i,l}}$, $l\in\{1, \ldots, p_i\}$ and
  $m_{i,l}$ denotes the dimension of $\ts_{i,l,j}$. 
  %Define
  %$\Phi_{i,l}=[\phi_{i,l,1}(\x)\ \cdots\ \phi_{i,l,m_{i,l}}]^T$. 
  %With
  %$\xi_{i,l}^t=D_{i_l}\Phi_{i,l}(\x^{(t)})$, 
  We can state \eqref{eq:y} as
  \begin{equation}
    \bmat{y_{i,1}^{k+1}\\ \vdots\\ y_{i,p_i}^{k+1}}=\bmat{(\xi_{i,1}^k)^T 
    &\cdots & 0\\
    % 0&(\xi_{i,2}^t)^T&0 &\cdots &0\\
     \vdots&  \ddots &\vdots\\
     0 &  \cdots  & (\xi_{i,p_i}^k)^T}\bmat{\ts_{i,1}\\ \vdots \\
     \ts_{i,p_i}} %+\bmat{w_{i,1}^{t+1}\\ \vdots\\ w_{i,p_i}^{t+1}}
    \label{eq:multi-in-1}
  \end{equation}
  In this case,   observations decouple and hence,
  the estimation for each set of parameters decouples. In this case, 
   each $\tit{i,l}{k}$ is updated  according to
  Algorithm~\ref{alg:nash} independently from the others.
  Since the notation is
  cumbersome and the details straightforward, we drop the additional index for
  each input. That is, instead of considering the update of our estimate of
  $\ts_{i,l}$ in Algorithm~\ref{alg:nash}, we simply consider the update of
  $\ts_i$ and note that due to the independence of the parameters for each
  input, that we could apply the update to each $\ts_{i,l}$.

  In addition, we will consider \emph{noisy} updates given by
%That is, we will denote each agent's update by $y_i^{t+1}$ where
\begin{equation}
  y_i^{k+1}=(\xi_i^k)^T\ts_i + w_i^{k+1}
  \label{eq:update-n}
\end{equation}
for each $i\in\pl$ where $w_i^{k+1}$ is an indepdent, identically distributed (i.i.d) 
%zero mean
real stochastic process defined on a probability space $(\Omega, F, P)$ adapted
to the sequence of increasing sub-$\sigma$--algebras $(F_k, k\in \mb{N})$, where
$F_k$ is the $\sigma$--algebra generated by the set $\{y_i^t,
\ala{t}{i},
w_i^t, t\leq k\}$ and
such that the following hold:
%$\mb{E}[(w_i^{t})^2]=\sigma_i^2$.
\begin{equation}
  \mb{E}[w_i^{k+1}| F_k]=0\  \forall k;\  \mb{E}[(w_i^{k+1})^2| F_k]=
  \sigma^2>0 \  \text{a.s.}\  \forall k; \ \sup_t \mb{E}[(w_i^{k+1})^4| F_k]<+\infty\ \text{a.s.}
  \label{eq:zeromean}
\end{equation}
%and
%\begin{equation}
%  \mb{E}[(w_i^{t+1})^2| F_t]= \sigma^2>0 \ \ \text{a.s.}\  \forall\  t.
%  \label{eq:var}
%\end{equation}
%and
%\begin{equation}
%  \sup_t \mb{E}[(w_i^{t+1})^4| F_t]<+\infty\ \text{a.s.}
%  \label{eq:fourthorder}
%\end{equation}
 Note that $F_k$ is also the $\sigma$--algebra generated by
$\{y_i^t, \xi_i^t, t\leq k\}$ since $w_i^k$ can be deduced from $y_i^k$ and
$\xi_i^{k-1}$ through the relationship
$w_i^{k}=y_i^k-(\xi_i^{k-1})^T\ts_i$~\cite{kumar:1986aa}.

For simplicity, in this section we will assume that $X_i\subseteq\mb{R}^{p_i}$
with $p_i>1$ and that there is a different set of basis functions for each input as
described in~\eqref{eq:multi-in-1}.  We will also drop the additional index
corresponding to each input for each player since the same analysis can be
applied to each of the inputs seperately. That is, instead of considering $p_i$
different observations 
 $y_{i,l}^{k+1}=(\xi_{i,l}^k)^T\ts_{i,l} + w_{i,l}^{k+1}$ for
$l\in\{1, \ldots, p_i\}$
we will perform the analysis for $y_i^{k+1}=(\xi_i^k)^T\ts_i + w_i^{k+1}$ and
simply note that the same analysis holds for each input without carrying around
the extra index $l$.
%Please refer back to Section~\ref{subsec:UL-nash} for the Nash case and
%Section~\ref{subsec:UL-myopic} for the myopic case.
%
%We address the scenario in which the agents' updates are \emph{noisy}. 

%\begin{theorem}
%  Suppose that for
%  each $i\in\pl$, 
%  $\{w_i^{k}\}$ satisfies \eqref{eq:zeromean} and that Algorithm~\ref{alg:nash},
%  with prox--mapping $P_\theta$ associated with $\beta$ (modulus $\nu$), is 
%  {persistently exciting} and stable.
%%  . Furthermore,
%%  suppose that a central planner follows Algorithm~\ref{alg:nash} for utility
%%  learning and incentive design using the 
%% prox--mapping $P_\theta$ associated with $\beta$ (modulus $\nu$)
%%  and that the algorithm is {persistently exciting} and stable. 
%Let the 
%  step--size $\eta_k$
%  be selected such that %$\sum_{t=1}^\infty \eta_t=\infty$,
%  $\sum_{k=1}^\infty\eta_k^2<\infty$ and
%  $\eta_k-\frac{\eta_k^2}{2\nu}\tilde{c}_1>0$
%  %for some $\vep$ such
%  %that $0<\vep <\frac{1}{2c_2}$ and 
%  where
%   $0<\tilde{c}_s<\infty$ is such that $\|\xi_i^k\|_\ast^2\leq \tilde{c}_s$.
%   %and
%   %$c_2=\min_{i\in\pl}c_{i,2}$.
%  Then, for each $i\in\pl$, 
%  $V_k(\ts_i)$ converges
%  {a.s}.
%  Furthermore, if the sequence
%  $\{r_k\}$ where $r_k=(\eta_k-\frac{\eta_k^2}{2\nu}\tilde{c}_s)^{-1}$ is a non-decreasing,
%  non-negative sequence such that $r_k$ is $F_k$ measurable and there
%  exists constants $0<K_1, K_2<\infty$ and $0<{T}<\infty$ such that
%  \begin{equation}\textstyle
%    \frac{1}{k}r_{k-1}\leq
%  K_1+\frac{K_2}{k}\sum_{t=0}^{k-1}(y_i^{t+1}-(\xi_i^{t})^T\tit{i}{t}-w_i^{t+1})^2,
%  \ \ \forall  \ k\geq {T},
%  \label{eq:rbound}
%\end{equation}
%then 
%\begin{equation}\textstyle
%  \lim_{k\rar\infty}
%  \frac{1}{k}\sum_{t=0}^{k-1}\mb{E}[(y_i^{t+1}-(\xi_i^{t})^T\tit{i}{t})^2|
%F_t]=\sigma^2\ \ \text{a.s.}
%\label{eq:errorcon-yy}
%\end{equation}
%  If, in addition,  
%  %\begin{equation}
%  $\sup_k \mb{E}[(w_i^{k+1})^4| F_k]<+\infty$ a.s.
%  %\label{eq:fourthorder}
%%\end{equation}
%then
%\begin{equation}\textstyle
%  \lim_{k\rar\infty}
%\frac{1}{k}\sum_{t=0}^{k-1}(y_i^{t+1}-(\xi_i^{t})^T\tit{i}{t})^2=\sigma^2\ \ \text{a.s.}
%\label{eq:errorcon-y}
%\end{equation}
%  %If, in addition,
%  %$\lim_{t\rar\infty}\left(\eta_t-\frac{\eta_t^2}{2\nu}\tilde{c}_1\right)^{-1}=\infty$,
%  %then 
%  %\begin{equation}
%  %  \lim_{T\rar\infty}\left( \eta_T-\frac{\eta_T^2}{2\nu}\tilde{c}_1
%  %  \right)\sum_{t=1}^T\left( \mb{E}[y_i^{t+1}-(\xi_i^t)^T\theta_i^{(t)}| F_t]
%  %  \right)^2=0 \ \ \text{a.s.}
%  %  \label{eq:limeq}
%  %\end{equation}
%  \label{thm:noise}
%\end{theorem}


%Before we move on, let us remark on the assumptions of Theorem~\ref{thm:noise}.
%We can make some modificaitons to the assumptions in order to simplify some of the
%ones that are more difficult to check. In particular, if we assume that each
%$\Theta_i^{(t)}$ is bounded, then by letting $r_t=\eta_t^{-1}$

%Let us state an alternative version of the above theorem after which we will make comments
%on the differences between the assumptions. 
\begin{theorem}
  Suppose that for
  each $i\in\pl$, 
  $\{w_i^{k}\}$ satisfies \eqref{eq:zeromean} and that Algorithm~\ref{alg:nash},
  with prox--mapping $P_\theta$ associated with $\beta$ (modulus $\nu$), is 
  {persistently exciting} and stable. Let the 
  step--size $\eta_k$
  be selected such that %$\sum_{t=1}^\infty \eta_t=\infty$,
  $\sum_{k=1}^\infty\eta_k^2<\infty$ and
  $\eta_k>0$
  %for some $\vep$ such
  %that $0<\vep <\frac{1}{2c_2}$ and 
  where
   $0<\tilde{c}_s<\infty$ is such that $\|\xi_i^k\|_\ast^2\leq \tilde{c}_s$.
   %and
   %$c_2=\min_{i\in\pl}c_{i,2}$.
  Then, for each $i\in\pl$, 
  $V_k(\ts_i)$ converges
  a.s.
  Furthermore, if %suppose that each $\Theta_i^{t}$ is bounded and that 
  the sequence
  $\{r_k\}$ where $r_k=(\eta_k)^{-1}$ is a non-decreasing,
  non-negative sequence such that $r_k$ is $F_k$ measurable and there
  exists constants $0<K_1, K_2<\infty$ and $0<{T}<\infty$ such that
  \begin{equation}\textstyle
    \frac{1}{k}r_{k-1}\leq
  K_1+\frac{K_2}{k}\sum_{t=0}^{k-1}(y_i^{t+1}-(\xi_i^{t})^T\tit{i}{t}-w_i^{t+1})^2,
  \ \ \forall  \ k\geq {T},
  \label{eq:rbound-22}
\end{equation}
then 
\begin{equation}\textstyle
  \lim_{k\rar\infty}
  \frac{1}{k}\sum_{t=0}^{k-1}\mb{E}[(y_i^{t+1}-(\xi_i^{t})^T\tit{i}{t})^2|
F_t]=\sigma^2\ \ \text{a.s.}
\label{eq:errorcon-2}
\end{equation}
  If, in addition, 
  %\begin{equation}\textstyle
  $\sup_k \mb{E}[(w_i^{k+1})^4| F_k]<+\infty$ {a.s.}
 % \label{eq:fourthorder-2}
%\end{equation}
then
\begin{equation}\textstyle
  \lim_{k\rar\infty}
\frac{1}{k}\sum_{t=0}^{k-1}(y_i^{t+1}-(\xi_i^{t})^T\tit{i}{t})^2=\sigma^2\ \ \text{a.s.}
\label{eq:errorcon-22}
\end{equation}
  \label{thm:noise-p}
\end{theorem}
The proof follows a similar technique to that presented in~\cite[Chapter
13.4]{kumar:1986aa}; hence, we leave it to Appendix~\ref{app:proofs}. 
%Note that added the assumption that each $\Theta_i^{t}$ is bounded and the
%modified
% assumption on the sequence $r_t$. 
% The proof follows the same argument as the
% proof of Theorem~\ref{thm:noise}.
%\begin{proof}
%    The proof is essentially the same as above with some minor modifications.
%    %follows a similar technique to that presented in~\cite[Chapter
%  %13.4]{kumar:1986aa}.
% % Since $\ell(\theta)$ is convex, we have
% % \[\ell(\tit{i}{t})-\ell(\theta_i)\leq \nabla
% % \ell(\theta_i)(\ta{i}-\tit{i}{t})\]
% Starting from Lemma~\ref{lem:tvpmaps}, we have
% \begin{align}
%   \mb{E}[V_{t+1}(\ts_i)|F_t]&\leq
%   V_t(\ts_i)-\eta_t(\ts_i-\tit{i}{t})^T\xi_i^t(\mb{E}[y_i^{t+1}-(\xi_i^t)^T\tit{i}{t}|F_t])\notag\\
%   &\qquad+\frac{\eta_t^2}{2\nu}\|\xi_i^t\|_\ast^2\left((\mb{E}[y_i^{t+1}-(\xi_i^t)^T\tit{i}{t}|F_t]
%    )^2+\sigma^2\right)\\
% %   &\leq V_t(\theta_i)-\eta_t\left(
% %   (\theta_i-\theta_i^{(t)})^T\xi_i^t-\frac{\eta_t}{2\nu}\|\xi_i^t\|_\ast^2\mb{E}[y_i^{t+1}-(\xi_i^t)^T\theta_i^{(t)}|F_t]
% %   \right)\notag\\
% %   &\qquad
% %   \cdot\mb{E}[y_i^{t+1}-(\xi_i^t)^T\theta_i^{(t)}|F_t]+\frac{\eta_t^2}{2\nu}\|\xi_i^t\|_\ast^2\sigma^2\\
%    &\leq V_t(\ts_i)-
%    \eta_t \left( \mb{E}[y_i^{t+1}-(\xi_i^t)^T\tit{i}{t}|F_t]
%    \right)^2\notag\\
%    &\qquad+\frac{\eta_t^2}{2\nu}\|\xi_i^t\|_\ast^2\left(\sigma^2+(\mb{E}[y_i^{t+1}-(\xi_i^t)^T\tit{i}{t}|F_t])^2
%    \right)
%%    &\leq  V_t(\theta_i)-\left(
%%    \eta_t-\frac{\eta_t^2}{2\nu}\tilde{c}_1 \right)\left( \mb{E}[y_i^{t+1}-(\xi_i^t)^T\theta_i^{(t)}|F_t]
%%    \right)^2+\frac{\eta_t^2}{2\nu}\tilde{c}_1\sigma^2
%   \label{eq:noiseeq}
% \end{align} 
% Hence, since $\Theta_i^{t}$ is bounded along with the stability assumption, we have that there exists some
% constant $b$ such that $\mb{E}[y_i^{t+1}-(\xi_i^t)^T\tit{i}{t}|F_t]<b$. 
%This gives us that 
%\eq{eq:r}{\mb{E}[V_{t+1}(\ts_i)|F_t]\leq V_t(\ts_i)-
%    \eta_t \left( \mb{E}[y_i^{t+1}-(\xi_i^t)^T\tit{i}{t}|F_t]
%    \right)^2+\frac{\eta_t^2}{2\nu}\|\xi_i^t\|_\ast^2\left(\sigma^2+b^2
%    \right)}
%
% By the assumptions that $\eta_t>0$ and
% $\sum_{t=1}^\infty\eta_t^2<\infty$, we can apply the almost supermartingale
% convergence theorem (Theorem~\ref{thm:asmc}) to get that  
% \begin{equation}\textstyle
% \sum_{t=1}^\infty 
%    \eta_t \left( \mb{E}[y_i^{t+1}-(\xi_i^t)^T\tit{i}{t}|F_t]
%    \right)^2<\infty\ \ \text{a.s.}
%    \label{eq:sumit-p}
%  \end{equation}
%     and that $V_t(\ts_i)$
%    converges almost surely. 
%  
%    The remainder of the proof follows exactly what was shown for
%    Theorem~\ref{thm:noise} only with $r_t=\eta_t^{-1}$; hence, we refer the reader to its proof.
%    %which is to say that $\|\theta_i^{(t)}-\theta_i\|^2$
%    %converges almost surely.
% \end{proof}
 \begin{corollary}
   Suppose the assumptions of Theorem~\ref{thm:noise-p} hold with the exception that in
   Algorithm~\ref{alg:nash}, we use the prox--mapping $P_\theta$ associated with
   $\beta(\theta)=\frac{1}{2}\|\theta\|_2^2$ (modulus $\nu=1$). Then 
   $V_k(\ts_i)=\frac{1}{2}\|\ts_i-\tit{i}{k}\|_2^2$ converges a.s.
  \label{cor:tscon}
 \end{corollary}

In the myopic--play case,
%---that is where
%  $\bx{i}{k+1}=\td{\Phi}_i(\xx{k})^T\ts_i+\td{\Psi}_i(\xx{k})^T\ala{k}{i}$---
  as
  a consequence of \eqref{eq:errorcon-2}, we expect that the average mean square error
  between the desired response $x^d$ and the actual response $\xx{k}$
  converges to $\sigma^2$ a.s. Indeed,
  %~\eqref{eq:errorcon-2} of
  %Theorem~\ref{thm:noise-p} implies  
\begin{align}\textstyle
%  &\lim_{T\rar\infty}
%  \frac{1}{T}\sum_{t=0}^{T-1}\mb{E}[(u_i^{(t+1)}-\td{\Psi}_i(u^{(t)})^T\alpha^{(t)}+w_i^{t+1}-u_i^d+\td{\Psi}_i(u^{(t)})^T\alpha^{(t)})^2|
%F_t]\\
%&\quad=
\lim_{k\rar\infty}\frac{1}{k}\sum_{t=0}^{k-1}\mb{E}[(\bx{i}{t+1}+w_i^{t+1}-x_i^d)^2|
F_t]
=\sigma^2\ \ \text{a.s.}
\end{align}
    Furthermore, note that we have designed
    $\ala{t+1}{i}$ to satisfy $\gamma_i(x^d)=\Psi(\xx{t})^T\ala{t+1}{i}$
  (or at the very least approximately if we solve the optimization problem posed
  in \eqref{eq:lsq-alpha-myop} as opposed to explicitly solving the linear
  system of equations). 
  
  On the other hand, in the Nash--play case, it is
  difficult to say much about the observed Nash equilibrium except in
  expectation. In particular, we can consider a modified version of
  Theorem~\ref{thm:nash-bound} where we consider the differential game form in
  expectation, i.e.~at iteration $k$,  the
  differential game form for the induced game is %given by
  \eq{eq:modomega}{\textstyle
  \td{\omega}(\theta,
  x)=\sum_{i=1}^\n\mb{E}\left[D_i\Phi_i(x)^T\theta_i+D_i\Psi_i(x)^T\ala{k}{i}+w_i^{k+1}|
  F_{k-1}\right].
%  \mb{E}\left[\sum_{i=1}^{\n}\sum_{l=1}^{p_i}\left(\sum_{j=1}^{m_i}D_{i_l}\phi_{i,j}(\x)\theta_{i,j}+\sum_{k=1}^{n_i}D_{i_l}\psi_{i,k}(\x)\alpha_{i,j}\right)
%   d\x_i^l\right]
  }
%  Before, we knew that $D_2\omega(\ts, x^d)$ was an isomorphism since $x^d$
%  is a non--degenerate differential Nash equilibrium. Here, in order to apply
%  the Implicit Function Theorem as in  Theorem~\ref{thm:nash-bound}, we need
%  that $D_2\td{\omega}(\ts, x^d)$ is an isomorphism. Hence, we have the
%  following result.
  
\begin{proposition}
  Suppose that $D_2\td{\omega}(\theta, x^d)$ is an isomorphism. There exists an
  $\epsilon>0$, such that for all $\tu{t}\in B_\epsilon(\ts)$,
   \begin{equation}
     % \|\x^{(t+1)}-\x^d\|\leq C\cdot M\|\theta^{(t+1)}-\theta\|
     \|x^{\ast}-x^d\|\leq  \left( \sup_{0\leq \lambda\leq 1}\|Dg(
     (1-\lambda)\ts+\lambda\tu{t})\| \right)\|\tu{t}-\theta\|
      \label{eq:bound-vep-noise}
    \end{equation}
    where
    %\begin{equation}\textstyle
      $Dg(\ts)=-(D_2\td{\omega})^{-1}(\ts, x^d)\circ D_1\td{\omega}(\ts, x^d)$.
    %  \label{eq:DG-noise}
    %\end{equation}
    and $x^\ast$ is a Nash equilibrium of the incentivized game  $(\fg{1}(x;
    \ts_1), \ldots, \fg{\n}(x, \ts_\n))$ with
    $\gamma_i(x)=\Psi_i(x)^T\ala{t}{i}$ for each $i\in\pl$. 
Furthermore, 
    if $\|Dg(\ts)\|$
 is uniformly bounded by $M>0$ on $B_{\epsilon}(\ts)$, then
    \begin{equation}
     % \|\x^{(t+1)}-\x^d\|\leq C\cdot M\|\theta^{(t+1)}-\theta\|
     \|x^{\ast}-x^d\|\leq  M\|\tu{t}-\ts\|
      \label{eq:bound-vep-n}
    \end{equation}
    \label{prop:noisynashbdd}
\end{proposition}
%As before, if the cost functions are convex and the incentive parameter $\alpha^{(t)}$ is chosen such
%that $u^{d}$ is a non--degenerate differential Nash equilibrium of the
%incentivized game and such that each $\fg{i}$ is convex,
%then we can replace $u^\ast$ with $u^{(t+1)}$ since $u^{(t+1)}$ is unique. 
%  \textcolor{red}{put in part about expected value theorem (need $E[\omega]$ to
%  be differentiable), also add in proof of contracting proximal map, and
%  consider mentioning the constant value version of the IFT}

%To apply Proposition~\ref{prop:noisynashbdd} we need
%that the parameter estimate $\tu{t}$ converges to the true parameter value
%$\ts$. One of the consequences of Theorem~\ref{thm:noise} (respectively
%Theorem~\ref{thm:noise-p}) is that $V_t(\ts_i)$ converges a.s.~and
%as a consequence of Corollary~\ref{cor:tscon}, $\|\ts_i-\tit{i}{t}\|_2^2$
%converges a.s. If the value it converges a.s. to is less than $\epsilon$,
%then Proposition~\ref{prop:noisynashbdd} would guarantee that a Nash
%equilibrium of the incentivized game is near the desired
%non--degenerate differential Nash equilibrium in expectation. We leave further
%exploration of the convergence of the parameter estimate $\tu{t}$ as
%future work. 

The results of Theorem~\ref{thm:noise-p}  imply  that the average mean square error
  between 
  the observations and the predictions converges to $\sigma^2$ a.s.~and
  if we recall, the observations are derived from noisy versions of the
  first--order conditions for Nash. Indeed,
%  i.e.~we have the observation
%  $y_i^{t+1}=(\xi_i^t)^T\ts_i+w_i^{t+1}=D_i\Phi_i(\xx{t+1})^T\ts_i+w_i^{t+1}$
%  and its predicted value
%  $(\xi_i^t)^T\tit{i}{t}=D_i\Phi_i(\xx{t+1})^T\tit{i}{t}=-\D_i\Psi_i(\xx{t+1})^T\ala{t}{i}.$
%  Thus,  
we have shown that
  \eq{eq:congverg1}{\textstyle\lim_{k\rar\infty}
  \frac{1}{k}\sum_{t=0}^{k-1}\mb{E}[(D_i\Phi_i(\xx{t+1})^T\ts_i+w_i^{t+1}+\D_i\Psi_i(\xx{t+1})^T\ala{t}{i})^2|
  F_t]=\sigma^2\ \ \text{a.s.}}
or, equivalently,
\eq{eq:converge2}{\textstyle\lim_{k\rar\infty}
\frac{1}{k}\sum_{t=0}^{k-1}\mb{E}[(D_i\Phi_i(\xx{t+1})^T(\ts_i-\tit{i}{t})+w_i^{t+1})^2|
F_t]=\sigma^2\ \ \text{a.s.}}

%Depending on the noise characteristics, particularly the magnitude of
%$\sigma^2$, we may be able to argue that the agents are playing an $\vep$--Nash
%equilibrium by using a similar argument to that in Theorem~\ref{thm:nash-bound}.
%The details are left for future work. In the concluding chapter, remarks will be
%made regarding the many open questions this work has exposed including making
%connections between traditional tools of adaptive control and online learning.
%which we will now make remarks about in the context of the previous sections of
%this chapter.
%Furthermore, we will cover the

% \end{remark}
%\begin{remark}[Connections to Adaptive Control and Online Learning]
%  There are some not so subtle connections to the adaptive control literature.
%  In particular, if in the myopic--play case the entries of
%  $\td{\Phi}_i(u)$ and $\td{\Psi}(u)$ are linear in $u_i$, then the problem can
%  easily as a classical linear adaptive control problem~\cite[Chapter 10 \& 13]{kumar:1986aa}.  The
%  Nash--play case has some distinctions in that the actual response is defined
%  implicitly through the first{\ds} and second{\ds}order conditions for local Nash
%  equilibria and is therefore new. 
%
%  Similarly, if we consider only the problem of estimating $\theta$, then both
%  the Nash--play case and the myopic--play case, even with nonlinearities in the
%  observation updates,
%  can be cast as online estimation
%  problem~\cite[Chapter 3 \& 8]{goodwin:1984aa} with the added difference
% that in the present work
%  we did not select specific step--sizes. For example, 
%%  \[\td{\Phi}_{i}(u)=[\td{\phi}_{i,1}(u)\ \cdots \td{\phi}_{i,m_i}(u)]\
%%  \text{ and } \td{\Psi}_{i}(u)=[\td{\psi}_{i,1}(u)\ \cdots \td{\psi}_{i,n_i}(u)]\]
%%  where $\td{\phi}_{i,j}(u)$ and $\td{\psi}_{i,j}(u)$ are linear in $u_i$
%%  the entire theory developed for the mu
%if we make specific choices for the step--size $\eta_t$ such as
%%$\eta_t=\frac{a}{c+\|\xi_i^t\|_\ast^2}$, then the assumptions of
%%Theorem~\ref{thm:noise} can be streamlined. For instance, using the $2$--norm so
% \[\eta_t=\frac{a}{c+\|\xi_i^t\|_2^2},\] the update scheme for
%$\theta^{(t)}_i$ reduces to the projection algorithm.
%Alternatively, if $\eta_t=\frac{\mu}{r_k}$ where
%$r_k=1+\sum_{t=0}^k(\xi_i^t)^T\xi_i^t$ and $\mu>0$, then updates for $\theta$
%follow the
%algorithm introduced in~\cite{kumar:1986aa}. 
%
%It is interesting
%to note that the persistence of excitation
%condition required to ensure convergence is informed by the choice of
%step--size. This is explored extensively in~\cite[Chapter 3.4]{goodwin:1984aa}.
%However, because the conditions required for persistence of excitation depend on
%the data received at each time step (and this is true of
%Definition~\ref{def:persist} as well), it is difficult to check when an
%algorithm is persistently exciting a priori.
%In~\cite{sastry:1989aa} and~\cite{boyd:1986aa}, necessary and sufficient
%conditions are provided for persistence of excitation for model reference
%adaptive control. We are exploring extensions for the problems described in
%this chapter.
%
%Our approach here is to try to remove the dependence of the results on the
%choice of step--size and to generalize to arbitrary choice of proximal mapping.
%This approach is similar to that which is done in 
%the online learning literature~\cite{raginsky:2010aa,
%nemirovski:2009aa}. The perceived gain is that this flexibility can allow for
%the proximal mapping to be informed by the geometry of the constraint set
%(feasible parameter space) thereby resulting in improved convergence rates. 
%
%There are a number of open questions in this area.
%For instance, in order to ensure we have estimated parameters that correspond
%to a game with stable, non--degenerate differential Nash equilibria requires
%having a constraint set defined by semi--definite constraints, i.e.
%\eq{eq:thetanew}{
%\Theta_i^k=\{\theta_i\in \Theta_i|\ D^2\Phi(u^{(t)}, \theta_i)+D^2\Psi(u^{(t)},
%\alpha^{(t-1)})\geq 0, \ t\in\{1, \ldots, k\}\}\subset \Theta_i}
%where $D^2\Phi$ and $D^2\Psi$ are defined in \eqref{eq:dsqphi} and \eqref{eq:dsqpsi}
%respectively. Given that proximal maps informed by the geometry---as the
%example in Remark~\ref{rem:geom} indicates---one interesting direction for future research is
%to investigate proximal maps that are 
%%Is there a
%%proximal map that is 
%informed by the geometry of a the positive semi--definite
%cone of matrices.
%%that leads to better, in some sense, convergence properties? We
%%leave such questions as future work.
%%which is commonly used in the adaptive
%%control literature and estimation~\cite{raginsky:2010aa}and some remarks on
%%  connection to adative control
%\end{remark}



==> incent_util_1.tex <==
%\section{Utility Learning Formulation}
%\label{sec:utillearn}



We first formulate the utility learning problem for both the {\nplay} and
{\mplay} cases  with the goal of placing both cases into a unified framework that we
can then use to define an algorithm for updating the estimate of
$\ts=(\ts_1, \ldots, \ts_\n)$
at each iteration.


\subsection{Utility Learning Under Nash--Play}
\label{subsec:UL-nash}
We assume that the {\coordinator} knows the parametric structure of the agents'
nominal cost functions
and receives observations of the agents' choices over
time.
%; however, it does not know the parameters of the agents' nominal cost functions. In
%particular, 
That is, for each $i\in\mc{I}$, we assume that the nominal cost function of agent $i$
has the form
\begin{equation}\textstyle
  f_i(x)=\sum_{j=1}^{m_i} \phi_{i,j}(x)\ts_{i,j} =\la \Phi_i(x),\theta_i^\ast\ra
  \label{eq:parametric}
\end{equation}
where each
$\phi_{i,j}\in C^2(X, \mb{R})$ is Lipschitz continuous and $\{\phi_{i,1}, \ldots,
\phi_{i,m_i}\}$ is the set of basis functions for player $i$.
%---that is,
%there exists a constant $K\geq 0$ such that for all $x,x'\in X$,
%\[ |\phi_{i,j}(x)-\phi_{i,j}(x')|\leq Kd_X(x,x')\]
%where $d_X$ is the usual Euclidean metric on $X$.
%
The basis
functions are known to the coordinator; however, the parameters $\ts_{i,j}$ are
unknown. 
%\begin{align}
%    \mc{F}_\phi=\{\phi_{i,j}\in C^2|~
%    |\phi_{i,j}(x)-\phi_{i,j}(x')|\leq Kd_X(x,x')\}
%    \label{<++>}
%\end{align}<++>

Let  $\mc{F}_\phi$ denote the set of $C^2$--\emph{Lipschitz continuous} basis
functions $\phi_{i,j}$
%for the agents' cost functions be denoted by
% , that is $\phi_{i,j}\in\mc{F}_\phi$ where $\phi_{i,j}:X\rar\mb{R}$ for each $j\in \{1, \ldots, m_i\}$ for
  %all $i\in \pl$.   
  Note that since elements of $\mc{F}_{\phi}$ are $C^2$--\emph{Lipschitz continuous}, the derivative of any function
  in $\mc{F}_\phi$ is uniformly bounded.

Define $\Phi_i(x)=[\phi_{i,1}(x)\ \cdots \ \phi_{i,m_i}(x)]^T$ and
$\ts_i=[\ts_{i,1}\ \cdots\ \ts_{i, m_i}]^T$. The admissible
set of parameters for player $i$ is denoted by $\Theta_i$, a compact
subset of $\mb{R}^{m_i}$. We will use the notation $f_i(x;\theta)$ and $\fg{i}(x; \theta)$ when we need to 
make the dependence on the parameter
$\theta$ explicit. 

Note that we are limiting the problem of asymmetric information to
one of \emph{adverse selection}~\cite{bolton:2005aa} since it is the parameters
of the cost functions (or update functions) that are unknown to the coordinator.

Let the admissible set of incentive mappings
$\Gamma\subset C^2(X, \mb{R})$ be all such mappings 
\begin{equation}\textstyle
  \gamma_i(x)=\sum_{j=1}^{\sn_i} \psi_{i,j}(x)\g_{i,j}
  \label{eq:gammaparam}
\end{equation}
for a set of basis functions $\{\psi_{i,1}, \ldots, \psi_{i,\sn_i}\}$ where
each $\psi_{i,j}\in C^2(X, \mb{R})$ and
$\g_i^T=[\g_{i,1}\ \cdots\ \g_{i,\sn_i}]$ are parameters. Let $\mc{F}_\psi$ be
the set of $C^2$--\emph{Lipschitz continuous} basis functions for the incentive
mapping. We use the notation
$\Psi_i(x)=[\psi_{i,1}(x)\ \cdots \ \psi_{i,\sn_i}(x)]^T$ and
we denote the collection of all parameters by $\alpha_i=[\alpha_{i,1} \ \cdots \
\alpha_{i,s_i}]^T$.

\begin{remark}
 This framework encompasses the case where the basis functions of
all the agents' cost functions are identical ($\phi_{i,j}\equiv\phi_j$, $\forall \
i\in\{1, \ldots, \n\}$), the basis functions of the incentive mappings for all
the agents are
identical ($\psi_{i,j}\equiv\psi_j$, $\forall \ i\in\pl$), or even
the case when the parameters of the incentive mappings are constrained to be
identical ($\alpha_{i,j}=\alpha_j$, $\forall \ i\in\pl$).  \hfill$\square$
\end{remark}




At each iteration the coordinator receives the collective response from the
agents, i.e. $x^k=(x_1^k, \ldots, x_n^k)$ at iteration $k$, and has the 
incentive parameters that were issued 
i.e.~$\alpha^k$ at iteration $k$. Each of the observations is assumed to be a Nash equilibrium.
 We denote the set of
observations up to time $k$ by $\{\xx{t}\}_{t=0}^{k+1}$---where $x^0$ is the
observed Nash equilibrium of the nominal game (without incentives)---and the set of incentive
parameters~$\{\alpha^t\}_{t=0}^k$. %For iteration $k$, 
%At iteration $k$, the coordinator has


%At iteration $k$, given $\{\xx{t}\}_{t=1}^{k+1}$---assumed
%to be Nash equilibrium---and
%$\{\al{t}\}_{t=0}^{k}$, the planner forms an estimate 
%$\tit{i}{k}$ for each $i\in \pl$. 
%Our goal is to formulate an online algorithm to estimate
%$\ts_i$ for each $i\in\pl$ as each new observation $\x^{(t)}$
%%---assumed to
%%be a Nash equilibrium---
%is received. The observations $u^{(t)}$ are assumed to be Nash equilibria.
%we get new observations
% 
%To this end, we write the problem in a more generic form. 

For the incentivized game
$(f_1^{\gamma_i}, \ldots, f_\n^{\gamma_\n})$, $D_i\fg{i}(x)=0$ and
$D_{ii}^2\fg{i}(x)\geq 0$ for each $i\in\pl$ are necessary conditions for a Nash equilibrium
$x$~\cite[Proposition~1]{ratliff:2015aa}. By assumption, each $\xx{k+1}$ is a Nash
equilibrium so that
%for each $t\in\{0,
%\ldots, k\}$, we have that 
\begin{equation}
  0_{p_i\times
  1}=D_i\fg{i}(\xx{k+1})={D_i\Phi_{i}(\xx{k+1})^T}\ts_i+{D_i\Psi_{i}(\xx{k+1})^T\ala{k}{i}}
  \label{eq:zero-cond-nash}
\end{equation}
where $D_i\Phi_{i}(\xx{k+1})=[D_{i_1}\Phi_i(\xx{k+1})\ \cdots \
D_{i_{p_i}}\Phi_i(\xx{k+1})]$ and we define $D_i\Psi_i(\xx{k+1})$ similarly.
%\[D_i\Phi_{i}(x^{(t+1)})^T=\bmat{D_{i_1}\Phi_i(x^{(t+1)})^T\\ \vdots\\
%D_{i_{p_i}}\Phi_i(x^{(t+1)})^T}.\]
In addition, for each $i\in \pl$, we have
 \begin{align}
   0&\leq D_{ii}^2\fg{i}(\xx{k+1})=D_{ii}^2\Phi_i(\xx{k+1},
   \ts_i)+D_{ii}^2\Psi_i(\xx{k+1}, \ala{k}{i})
   \label{eq:secondord-cond}
 \end{align}
  where
  \begin{equation}
    D_{ii}^2\Phi_i(\xx{k+1},
   \ts_i)=\bmat{D_{i_1i_1}^2\Phi_i(\xx{k+1})^T\ts_i
   & \cdots & D_{i_{p_i}i_1}^2\Phi_i(\xx{k+1})^T\ts_i\\
   \vdots & \ddots & \vdots\\
   D_{i_1i_{p_i}}^2\Phi_i(\xx{k+1})^T\ts_i &\cdots &
   D_{i_{p_i}i_{p_i}}^2\Phi_i(\xx{k+1})^T\ts_i}
   \label{eq:dii-phi}
 \end{equation}
 and $D_{ii}^2\Psi_i(\xx{k+1}, \ala{k}{i})$ is defined similarly.
%\begin{equation}
%  D_{ii}^2\Psi_i(x^{(t+1)}, \alpha_i^{(t)})=\bmat{D_{i_1i_1}^2\Psi_i(x^{(t+1)})^T\alpha_i^{(t)}
%& \cdots & D_{i_{p_i}i_1}^2\Psi_i(x^{(t+1)})^T\alpha_i^{(t)}\\
%   \vdots & \ddots & \vdots\\
%   D_{i_1i_{p_i}}^2\Psi_i(x^{(t+1)})^T\alpha_i^{(t)} &\cdots &
%   D_{i_{p_i}i_{p_i}}^2\Psi_i(x^{(t+1)})^T\alpha_i^{(t)}}.
%   \label{eq:dii-psi}
% \end{equation}
%%In an effort to unify notation across the Nash--play and myopic--play cases,  we 

Let $\Theta_i\subset \mb{R}^{m_i}$ be the set of \emph{admissible parameters} 
for agents $i$. We assume $\Theta_i$ is compact %We make the following assumption:
%\begin{assumption}
 and that for each $i\in\mc{I}$, $\ts_i\in \Theta_i$, i.e.~each agent's true
  parameters are in the admissible set. % \hfill$\square$
%\end{assumption}
Let the admissible set of $\theta_i$'s at iteration $k$ be denoted by
$\Theta_i^{k}$. They are defined using the second--order
conditions from the assumption that the observations at times $t\in\{1, \ldots,
k\}$ are Nash equilibria and are
%To make this more concrete, consider the case where each $p_i=1$, $i\in\pl$.
%Then we can define 
%\begin{equation*}
%  A_i(\xx{1,k})=\bmat{D_{ii}^2\Phi_i(\xx{1})^T\\ \vdots \\
%  D_{ii}^2\Phi_i(\xx{k})^T} \ \text{and } \
%  b_i(\xx{1,k}, \ala{0,k-1}{i})=\bmat{D^2_{ii}\Psi_i(x^{(1)})^T \alpha_i^{(0)}\\ \vdots
%  \\ D^2_{ii}\Psi_i(x^{(k)})^T
%  \alpha_i^{(k-1)}}
%\end{equation*}
%where we use the fact that $D_{ii}^2\Phi_i(x^{(t)}, \ts_i)=D_{i_1
%i_1}^2\Phi_i(x^{(t)})^T\ts_i=D_{i
%i}^2\Phi_i(x^{(t)})^T\ts_i$ and we use the notation $\xx{1,k}=(\xx{1}, \ldots, \xx{k})$ and similarly
%for $\ala{0,k-1}{i}$.
%Then using the above notation, the set of admissible $\theta_i$'s are defined
%by
%\begin{equation}
%  {\Theta}^{k}_i=\{\theta_i\in \Theta_i|\ A_i(\xx{1,k})\theta_i+b_i(\xx{1,k},
%  \ala{0,k-1}{i})\geq
%0\}\subseteq \Theta_i.
%  \label{eq:thetas}
%\end{equation}
%%Then the set of 
%% pretty sure these are closed and thus compact\ldots
%%Note that ${\Theta}^{(k)}_i\subseteq  {\Theta}_i^{(k-1)}\subseteq \cdots
%%\subseteq  {\Theta}_i^{(0)}\subseteq \Theta_i$. 
%%Thus, it is clear that the sets are nested. 
%Similarly, for higher dimensional
%strategy spaces, i.e. $p_i>1$, 
given by
\begin{equation}
  {\Theta}^{k}_i=\{\theta_i\in \Theta_i|\
  D_{ii}^2\Phi_i(\xx{t},\theta_i)+D_{ii}^2\Psi_i(\xx{t},
  \ala{t-1}{i})\geq
  0, t\in\{1,\ldots, k\}\}\subseteq \Theta_i.
  \label{eq:thetak-2}
\end{equation}
These sets are nested, i.e.
 ${\Theta}^{k}_i\subseteq  {\Theta}_i^{k-1}\subseteq \cdots
\subseteq  {\Theta}_i^{0}\subseteq \Theta_i,$
 since at each iteration an additional constraint is added
 to the previous set.
Note, the sets are defined by semi{\ds}definite constraints which are 
convex~\cite{boyd:2004aa}.
%where we use the notation 
Moreover, $\ts_i\in
\Theta_i^{k}$ for all $k$ since, by assumption, each observation $\xx{k}$ is
a local Nash equilibrium.

Let 
$y_i^{k+1}=-D_i\Psi_i(\xx{k+1})^T\ala{k}{i}$
and define
$\xi_i^k=D_i\Phi_i(\xx{k+1})$ 
%\eq{eq:ydef-np}{y_i^{t+1}=-D_i\Psi_i(x^{(t+1)})^T\ala{t}{i}} and
%\eq{eq:regdef-np}{\Xi_i^t=D_i\Phi_i(x^{(t+1)})} 
so that
\begin{equation}
  y_i^{k+1}=(\xi_i^k)^T\ts_i.
  \label{eq:y}
\end{equation}
Then, the coordinator has observations $\{y_i^t\}_{t=1}^{k+1}$ and \emph{regression
vectors} $\{\xi_i^t\}_{t=1}^{k}$.
We use the notation $\xi^k=(\xi_1^k, \ldots, \xi_n^k)$ for the regression
vectors of all the agents at iteration $k$.
\subsection{Utility Learning Under Myopic--Play}
\label{subsec:UL-myopic}
As in the Nash--play case, we assume the coordinator knows the parametric
structure of the myopic update rule. That is to say, the nominal update function
$g_i$ is parameterized by $\theta_i$ over basis functions $\{{\phi}_{i,1},
\ldots, {\phi}_{i,s_i}\}$ and the incentive mapping ${\gamma}_{i}^k$
at iteration $k$ is parameterized by
$\alpha_i^k$ over basis functions
$\{{\psi}_{i,1}, \ldots, {\psi}_{i,n_i}\}$. Define
${\Phi}_i=[{\phi}_{i,1} \ \cdots \ {\phi}_{i,m_i}]^T\in \mb{R}^{p_i\times m_i}$ and
${\Psi}_i=[{\psi}_{i,1} \ \cdots \ {\psi}_{i,s_i}]^T\in
\mb{R}^{p_i\times s_i}$.
We define $\mc{F}_\phi$ and $\mc{F}_\psi$ to be the set of $C^2$--\emph{Lipschitz continuous}
objective and incentive basis functions respectively, as before.
%for the agents' cost functions be denoted by
%  , that is $\phi_{i,j}\in\mc{F}_\phi$ where $\phi_{i,j}:X\rar\mb{R}$ for each $j\in \{1, \ldots, m_i\}$ for
%  all $i\in \pl$. 
We
assume the coordinator observes the initial response $x^0$ and we denote
the past responses up to iteration $k$ by $x^{(0,k)}=(x^0,\ldots, x^k)$.
The myopic update rule is given by
\begin{equation}
  \bx{i}{k+1}=g_i^{{\gamma_i}}(\bx{i}{(0,k)},
 \bx{-i}{(0,k)})={\Phi}_i(\bx{i}{(0,k)},
  \bx{-i}{(0,k)})^T\theta_i^\ast+{\Psi}_i(\bx{i}{(0,k)},
  \bx{-i}{(0,k)})^T\ala{k}{i}.
  \label{eq:myopic_update}
\end{equation}
Note that the update rule does not need to depend on the whole sequence of past
response. It could depend just on the past response $x^k$ or a subset, say
$x^{(j,l)}$ for $0\leq j\leq l\leq k$.
As before, we denote the set of admissible parameters for player
$i$ by $\Theta_i$ which we assume to be a compact subset of $\mb{R}^{m_i}$.
%Again, we
%assume that $\ts_i\in \Theta_i$ for each $i\in\pl$. 
In contrast to the {\nplay} case, our admissible set  of
parameters is no long time varying so that $\Theta_i^k=\Theta_i$ for all $k$.

%Recall the myopic--play update rule given in \eqref{eq:myopic_update} for each
%$i\in\pl$ where $\td{\Phi}_i(\xx{k})^T\in \mb{R}^{p_i\times m_i}$ and
%$\td{\Psi}_i(\xx{k})^T\in\mb{R}^{p_i\times n_i}$. Note that $\td{\Phi}_i$ and
%$\td{\Psi}_i$ could on the entire past response which we denote by
%$\xx{(0,k)}$ or some subset of the past responses $\xx{(j,l)}$ for some
%$j,l\in\{0, \ldots, k\}$ such that $j\leq l$. 
Keeping consistent with the notation of the previous sections, we let
%\eq{eq:yup-mp}{
$\xi_i^k={\Phi}_i(\xx{k})$  and 
$y_i^{k+1}=\bx{i}{k+1}-{\Psi}_i(\xx{k})^T\ala{k}{i}$ 
%\eq{eq:regup-mp}{
so that \eqref{eq:myopic_update} can be rewritten as
%\begin{equation}
  $y_i^{k+1}=(\xi_i^k)^T\ts_i.$
Analogous to  the previous case, 
the coordinator has observations $\{y_i^t\}_{t=0}^{k+1}$ and regression
vectors $\{\xi_i^t\}_{t=0}^{k}$.
Again, we use the notation $\xi^k=(\xi_1^k, \ldots, \xi_n^k)$ for the regression
vectors of all the agents at iteration $k$. 

%  \label{eq:general-y-up}
%\end{equation}
%At iteration $k$, the {\coordinator}
%uses data $\{\xx{t}\}_{t=0}^{k+1}$ and $\{\al{t}\}_{t=0}^{k}$ to estimate
%$\tu{k}$ which is used to design $\al{k}$.
%Notice that we assume the
%coordinator observes $\xx{0}$---this was not needed in the Nash--play case.

\subsection{Unified Framework for Utility Learning}
In both the Nash--play and myopic--play cases, the coordinator has 
We can describe both the Nash--play and myopic--play cases in a unified
framework as follows. At iteration $k$, the coordinator receives a response
$x^{k+1}$ which lives in the set $\mc{X}_k(x^{(0,k)},
\theta^\ast,\alpha^k)$ which is either the set of Nash equilibria of the
incentivized game  or the unique response determined by the
incentivized myopic update rule at iteration $k$. The coordinator uses the past
responses $\{x^t\}_{t=0}^{k+1}$ and incentive parameters $\{\alpha^t\}_{t=0}^k$
to generate the set of observations $\{y^t\}_{t=0}^{k+1}$ and regression vectors
$\{\xi^t\}_{t=0}^k$. 

The utility learning problem is formulated as an online optimization problem in
which parameter updates are calculated following the gradient of a loss
function.
%At each iteration, the algorithm will have two main steps: update the estimate
%of $\theta_i$ and choose parameters $\alpha_i$. 
For each $i\in\pl$, consider
the loss function 
\eq{eq:loss_function}{\textstyle \ell(\tit{i}{k})=\frac{1}{2}(y^{k+1}_i-(\xi_i^k)^T\tit{i}{k})^2} 
that evaluates the error in the predicted observation and the true observation
at time $k$
for each player.

Before we describe the parameter estimate update step, let us first review some concepts from online optimization. Denote by $\partial f(x)$ the set of 
\emph{subgradients} for the function $f:X\rar\mb{R}$. A function $\beta:\Theta\rar\mb{R}$ is a \emph{distance
generating} function modulus $\nu>0$ with respect to $\|\cdot\|$, if
$\beta$ is convex and continuous on $\Theta_i$, the set 
$\Theta^\circ=\{\theta\in \Theta| \partial \beta(\theta)\neq
\emptyset\}$
is convex 
%($\Theta^\circ$ always contains the relative interior of $\Theta$)
and restricted to $\Theta^\circ$, $\beta$ is continuously differentiable and
\emph{strongly convex} with
parameter $\nu$ with respect to $\|\cdot\|$, that is
\eq{eq:strong_convexity}{(\theta'-\theta)^T(\nabla\beta(\theta')-\nabla\beta(\theta))\geq
\nu\|\theta'-\theta\|^2, \ \ \forall \ \theta', \theta\in \Theta^\circ.}
%As an example, consider $\beta(\theta)=\frac{1}{2}\|\theta\|_2^2$ (modulus
%$\nu=1$
%with respect to $\|\cdot\|_2$, $\Theta^\circ=\Theta$). 
A function $V:\Theta^\circ\times \Theta\rar \mb{R}_+$ satisfying
\begin{equation}
  V(\theta_1, \theta_2)=\beta(\theta_2)-\left(
  \beta(\theta_1)+\nabla\beta(\theta_1)^T(\theta_2-\theta_1) \right)
  \label{eq:Vdef-1}
\end{equation}
is a \emph{prox--function} (Bregman divergence~\cite{bregman:1967aa})
associated
with distance generating function $\beta(\theta)$. The function $V(\theta_1,
\cdot)$ is nonnegative and is a strongly convex modulus $\nu$ with respect to
$\|\cdot\|$. 
A mapping
 $P_{\theta}^k:\mb{R}^{m}\rar
(\Theta^{k})^{\circ}$ associated with $\beta$ and a point $\theta\in
(\Theta^{k})^\circ$ such that
\begin{equation}
  P_\theta^k(g)=\arg\min_{\theta'\in \Theta^{k}}\left\{
 g^T(\theta'-\theta)+V(\theta, \theta') \right\}.
  \label{eq:proxmap-def-theta}
\end{equation}
is a  \emph{time varying prox--mapping}. This mapping is well-defined and is a
contraction~\textcolor{red}{cite my lemma}.
%$P_{\theta}:\mb{R}^{m}\rar \Theta^\circ$ associated with $\beta$ and a point $\theta\in
%\Theta^\circ$ defined by
%\begin{equation}
%P_\theta(g)=\arg\min_{\theta'\in \Theta}\left\{
%  g^T(\theta'-\theta)+V(\theta, \theta') \right\}
%  \label{eq:proxmap-def}
%\end{equation}
%is a \emph{prox--mapping}.
%The prox--mapping is well--defined and 
%is a contraction~\cite[Proposition~5.b]{moreau:1965aa}.
%Similarly, we define a is 

%We denote by $\Pi_{\Theta}$ the metric projection operator onto the set $\Theta$,
%that is, 
%\begin{equation}
%  \Pi_{\Theta}(\theta)=\arg\min_{\theta'\in \Theta}\|\theta-\theta'\|_2.
%  \label{eq:projop}
%\end{equation}
%For $\beta(\theta)=\frac{1}{2}\|\theta\|_2^2$, we have that
%$P_{\theta}=\Pi_{\Theta}(\theta-\theta')$.
%Note that for $\beta(\theta)=\frac{1}{2}\|\theta\|_2^2$, we have $V(\theta,
%\theta')=\frac{1}{2}\|\theta-\theta'\|_2^2$, $\nu=1$,
%$\|\cdot\|_\ast=\|\cdot\|_2$.

%If the sets $\Theta^{(k)}$ are nests, i.e. $$\cdots \subseteq \Theta^{(k+1)}\subseteq \Theta^{(k)}\subseteq \cdots
%\subseteq \Theta^{(0)}\subseteq \Theta,$$ then it is straightforward to see that
%the time--varying prox--mapping
%is also a 
%contraction.


At iteration $k$, the parameter estimate of each $\theta_i$ is updated according to 
\begin{equation}
  \tit{i}{k+1}=P_{\tit{i}{k}}^{k+1}\left( \eta_k\nabla \ell(\tit{i}{k}) \right)
  \label{eq:theta_up_prox}
\end{equation}
where $P_{\tit{i}{k}}$ is a prox{\ds}mapping associated with a distance
generating function $\beta(\theta)$. 
We remark that in the myopic--play case, a time--varying prox--mapping is not
necessary and instead one can use the standard prox--mapping which is also
well--defined and a contraction~\cite[Proposition~5.b]{moreau:1965aa}.
Note that if the prox{\ds}mapping that is used is 
associated with the distance generating function $\beta(\theta)=
\frac{1}{2}\|\theta\|_2^2$, then the prox{\ds}mapping is the usual Euclidean
projection, 
$P_\theta(\theta')=\Pi_{\Theta_i}(\theta-\theta')$, so that
\begin{equation}
  \tit{i}{k+1}=\Pi_{\Theta_i^{k}}\left( \tit{i}{k}-\eta_k\nabla
  \ell(\tit{i}{k}) \right).
  \label{eq:theta_up}
\end{equation}


%The reason we need it in the myopic--play case is so we can determine $\Xi_i^0$
%and $y_i^{1}$. 
%Without reiterating the details, just as in  Section~\ref{subsec:UL-nash}, we
%can formulate an optimization problem to solve for each $\theta^{(t)}_i$ at
%iteration $t$ (see \eqref{eq:opttheta}). Again, we will formulate an online
%learning algorithm in lieu of solving a full optimization problem, albeit convex, at each step.

%Now we have massaged both the {\nplay} and {\mplay} cases in to the same basic
%form, i.e.~for each case, at iteration $k$, the coordinator receives an observation 
%\eq{eq:yobs-mp}{
%y_i^{k+1}=(\Xi_i^k)^T\ts_i
%}
%for each $i\in\pl$ and the coordinator's goal is to estimate $\ts_i$ given the past
%observations and the past incentives. 


%Now we state the optimization problem for the estimate of player $i$'s
%parameters $\theta_i^{(k)}$ at iteration $k$:
%\begin{equation}
%  \min_{\theta_i\in {\Theta}_i^{(k)}} J(Y_i^{k+1}-\Xi_0^k\theta_i) %\|Y_i^{k+1}-\Xi_0^k\theta_i\|_2^2
%  \label{eq:opttheta}
%\end{equation}
%where $J$ is a convex, real-valued loss function. For instance,
%$J(\cdot)=\|\cdot\|_2^2$. Our aim will be to formulate an online version of the
%above optimization problem which we will do in Section~\ref{subsec:alg-nash}.
%First, we formulate the incentive design problem.

%This would certainly be the case for an update rule
%determine by approximate fictitious
%play, for instance. In the remainder, we will simply show the dependence
%on $u^{(k)}$ and just remind the reader that the framework is flexible enough to
%encompass dependence on any subset of the past responses. 
%%where $\theta=(\theta_1, \ldots, \theta_\n)$ and $\alpha^{(k)}=(\ala{k}{1},
%%\ldots, \ala{k}{\n})$ as before. 
%%Further, $\tilde{\Phi}$ is a matrix--valued
%%mapping collectively representing the agents' core cost functions and
%%$\tilde{\Psi}$ is a matrix--valued mapping collective representing the
%%incentives. 
%Let us consider an example. Suppose the agents are playing according to gradient
%play. Then,
% for a given player's incentivized cost $\fg{i}(\x)=\Phi_i(\x)^T\ts_i+\Psi_i(\x)^T\alpha_i$
%it is straightforward
%to write 
%\[\x^{(k+1)}_i=\x^{(k)}_i-h_i(D_i\Phi_i(\x^{(k)})^T\ts_i+D_i\Psi_i(\x^{(k)})^T\alpha_i^{(k)})\]
%for each $i\in\pl$ in the form of \eqref{eq:update-gen-pl} by either augmenting
%the parameter $\ts_i$ to contain the observation $u_i^{(k)}$ at each iteration
%and modifying the constraint set for $\theta$ appropriately
%or by allowing the left{\ds}hand side of \eqref{eq:update-gen-pl} to be $\Delta
%u^{(k+1)}_i=(u_i^{(k+1)}-u_i^{(k)})$ and then defining $\td{\Phi}_i$ and
%$\td{\Psi}_i$ appropriately.
%We remark that the formulation of the update rule from the particular
%myopic{\ds}play details determines the relationship between
%$\gamma_i(\x)=\Psi_i(\x)^T\alpha_i$ and $\td{\Psi}_i(\x)$. For that matter, it
%also determines the relationship between $f_i$ and $\td{\Phi}_i$.
%%$\tilde{\Phi}_i^T$---the $i$--th row of $\td{\Phi}^T$---is given by
%%\[\td{\Phi}_i(\x)=[D_1\phi_{1,1}(\x)\ \cdots \ D_1\phi_{1,m_1}(\x)]\]
%%and $\td{\Psi}_i^T$---the $i$--th row of $\td{\Psi}^T$---is given by
%%\[\td{\Psi}(\x)^T=[D_1 
%
%%As before, we will denote player $i$'s strategy space by $\U_i\subset
%%\mb{R}^{l_i}$
%%and again remark that an extension to higher--dimenional strategy spaces can be
%%done provided some assumptions are made on the problem formulation as outlined
%%in Remark~\ref{rem:multi}. 
%; however, it could be time{\ds}varying in the event there are
%additional constraints that need to be enforced as long as the true parameter
%$\ts_i$ remains in the admissible set at each iteration and the sets remain closed.
%Our {\coordinator} will again have cost function $f_
%While we try to keep the notation consistent, we remark that there is a slight
%difference is the initial part of the utility learning and incentive design
%process for the myopic--play case as compared to the Nash--play case which results in a
%small indexing change. We suppose that the {\coordinator} issues $\alpha^{(-1)}$ and receives response
%$\x^{(0)}$ from the players. Using this information, the {\coordinator}
%estimates $\theta^{(0)}$ which is then, in turn, used to design $\alpha^{(0)}$
%such that it induces the desired output $\x^d$ while satisfying
%$\gamma(\x^d)=\Phi(\x^d)^T\alpha^{(0)}=\y^d$. This process repeats so that at
%The update rule for each individual player can be written as 
%\begin{equation}
%  \x^{(k+1)}_i=\tilde{\Phi}_i(\x^{(k)})^T\theta_i+\tilde{\Psi}_i(\x^{(k)})^T\alpha_i^{(k)}.
%  \label{eq:update-gen-i}
%\end{equation}



==> intro2.tex <==
In the emerging data market, classical learning and optimization tools no longer
suffice for efficient operations since data sources are often strategic in how
they respond to queries from system coordinators.

We will consider a class incentive design problems in which the  coordinator
does not know the underlying preferences, or decision--making process, of the agents that it is trying to coordinate. In the economics
literature these types of problems are known as problems of \emph{asymmetric
information}---meaning that the involved parties do not possess the same
information sets and, as is often the case, one party posses some information
 to which the other party is not privy.  The particular type of information
 asymmetry which we consider, i.e. where the preferences of the agents are
 unknown to the planner, results in a problem of \emph{adverse selection}~\cite{akerlof:1970aa}. 
 %The classic example of adverse selection is the \emph{market for
 %lemons}~\cite{akerlof:1970aa} in which the seller of a used car knows more
 %about the car than
 %the buyer. There are a number of components that are hidden from the buyer such
 %as the maintenance upkeep history, engine health, etc. Hence, the buyer could
 %end up with a \emph{lemon} instead of a \emph{cherry}.

 We assume that
agents, including the {\coordinator}, are cost minimizers or alternatively,
utility maximizers---while in this chapter we will formulate the entire problem
given all agents are cost minimizers, the utility maximization formulation is
completely analogous.
When we say the {\coordinator} does not know the underlying preferences of the
agents, we are assuming that it does not know the value of the parameters 
of the agents' cost functions. In the following sections, by taking a
non{\ds}Bayesian approach, we will formulate a utility learning and incentive design
problems for both the case when the agents play according to a Nash equilibrium as well as the
case when the agents play myopically---e.g.~the agents play according to a
myopic update rule. We formulate an algorithm for iteratively estimating
preferences and designing incentives. By adopting
tools from adaptive control and online learning, we show that the
algorithm converges under reasonable assumptions.

% by taking a non-Bayesian approach,

%The results in this have strong ties to both the adaptive control
%literature~\cite{goodwin:1984aa,kumar:1986aa,sastry:1989aa} and the online
%learning literature~\cite{cesa-bianchi:2006aa,nemirovski:2009aa,raginsky:2010aa}. The former gives us tools to do tracking of both the observed output
%(agents' strategies) and the control input (incentive mechanism). It also allows
%us to go one step further and prove parameter convergence under some
%additional assumptions---\emph{persistence of excitation}---on the problem formulation and, in particular, the
%utility learning and incentive design algorithm. The latter
%provides tools that allow us to generalize the algorithm and get faster
%convergence of the observed actions of the agents to a more desirable or even
%socially optimal outcome. 

The remainder of the paper is organized as follows. We first introduce the
problem formulation in Section~\ref{sec:formulation}. We follow that with
the \emph{utility learning} problem for both the case when the agents play according to
a Nash strategy and when they play myopically in Section~\ref{sec:utillearn}. We
formulate the incentive
design problem in Section~\ref{sec:incent-incent} again for both the case when
agents play Nash and when they play myopically. In Section~\ref{sec:alg}, we
present the utility learning and incentive design algorithm and study its
convergence in the case without noise in Section~\ref{subsec:converge-myopic} and with
noise in Section~\ref{sec:noise}. In Section~\ref{sec:examples}, we present
several simple, but illustrative, examples. Finally, we wrap up with discussion and future
directions in Section~\ref{sec:discussion}.
% Q for me: what happens if we take a non-bayesian approach to the privacy
% problem and we look at the solution to which we converge. do we get any
% interesting properties? is this basically the thing I was looking at?

%in the context of privacy-aware
%contract design for the demand-side of the smart grid. However, we will take a
%Bayesian approach 



==> makefile <==
# set latexfile to the name of the main file without the .tex
latexfile = 2017TACLT
# put the names of figure files here.  include the .eps
#figures = 
# if no references, run "touch latexfile.bbl; touch referencefile.bib"
# or delete dependency in .dvi and tarball sections
# referencefile = 2017TACLTrefs


TEX = pdflatex

# support subdirectories
VPATH = Figs

$(latexfile).pdf : $(figures) $(latexfile).tex 
#$(latexfile).dvi : $(figures) $(latexfile).tex $(latexfile).bbl
	while ($(TEX) $(latexfile) ; \
	grep -q "Rerun to get cross" $(latexfile).log ) do true ; \
	done


$(latexfile).tar.gz : $(figures) $(latexfile).tex
	tar -czvf $(latexfile).tar.gz $^

tarball: $(latexfile).tar.gz

cpall:
	make; skim $(latexfile).pdf

bib:
	bibtex $(latexfile)

clean:
	rm $(latexfile).dvi $(latexfile).log $(latexfile).ps $(latexfile).pdf

mpdf:
	pdflatex $(latexfile).tex; skim $(latexfile).pdf

